Anticipatory Mobile Computing: A Survey of the State of the Art and Research Challenges

Today's mobile phones are far from mere communication devices they were ten years ago. Equipped with sophisticated sensors and advanced computing hardware, phones can be used to infer users' location, activity, social setting and more. As devices become increasingly intelligent, their capabilities evolve beyond inferring context to predicting it, and then reasoning and acting upon the predicted context. This article provides an overview of the current state of the art in mobile sensing and context prediction paving the way for full-fledged anticipatory mobile computing. We present a survey of phenomena that mobile phones can infer and predict, and offer a description of machine learning techniques used for such predictions. We then discuss proactive decision making and decision delivery via the user-device feedback loop. Finally, we discuss the challenges and opportunities of anticipatory mobile computing.

==> tex/00_abstract.tex <==
\begin{abstract}
Today's mobile phones are far from mere communication devices they were ten years ago. Equipped with sophisticated sensors and high power computing hardware, mobile phones can be used to infer user's location, activity, social setting and more. As mobile devices become increasingly intelligent, their capabilities evolve beyond inferring context to anticipating it. In this article we provide an overview of the current state-of-the-art work in predictive mobile sensing. We present a survey of phenomena that mobile phones can infer and predict, and complement it with a description of machine learning techniques used for such predictions. Finally, we discuss the future of anticipatory pervasive computing, outlining the open challenges and a research agenda for the next years. %, specifically how can anticipated events can be used as a basis for smart decision making.
\end{abstract}



==> tex/01_introduction.tex <==
\section{Introduction}
%
%% Mobile sensing systems proliferation
%The ability to communicate on the move has revolutionized the lifestyle of millions of individuals: it changed the way we work, organize our daily schedules, develop and maintain social ties, enjoy our free time, and handle emergencies. In the last decade mobile phones have reached every part of the world, and 86\% of the world's population had a cellular subscription in year 2012 \cite{ITU2012}. 
%When smartphones replaced feature phones another mobile revolution has happened. Nowadays, phones serve for travel planning, staying in touch with online social network contacts, online shopping and numerous other purposes. Today's smartphones with multi-core CPUs and gigabytes of memory are capable of processing tasks that yesterday's desktop computers struggled with. However, unlike desktop computers, smartphones are small mobile devices. Consequently, phones became part of everyday life and remain continuously present and used at all times. In addition, modern-day smartphones host a variety of sophisticated sensors. Thus, a phone can sense its orientation, acceleration in three dimensions, location, and can record audio and video. As such, a smartphone is not just a mobile computer -- it is a perceptive device capable of extending human senses~\cite{Lane2010}. Finally, these devices are connected to the Internet and, therefore, they can share the data they collect and exploit the resources offered by cloud services.
%
%Despite the recent phenomenal progress, the area of mobile personal devices promises further advances as sensing and processing capabilities of mobile phones grow. We envisage mobile devices capable of full context awareness and intelligent reasoning based on the prediction of future events. Therefore, in this survey we summarize recent efforts in the area of \textit{anticipatory mobile computing}. 
%%Finally, we discuss the future of anticipatory pervasive computing, specifically: how anticipated events can be used as a basis for intelligent decision making.
%%
%%
%% From raw data to high level information
%
%Today's mobile devices can sense an abundance of information from the environment. However, rich streams of sensor data are seldom useful before significant data processing is employed. Just as detecting certain power levels at certain audio frequencies remains useless until our brain interprets sounds to speech, so does raw smartphone sensor data carry little value until it is used to infer high level concepts. Context sensing aims to reconstruct some key characteristics of the environment and human activities from sensed signals~\cite{Coutaz2005}. For that, in each of the domains, whether it is speech analysis, movement tracking, object recognition or any other domain, we need to identify features of raw signals that are useful to infer higher level concepts and characteristics. Machine learning techniques~\cite{Bishop2006} are widely used to extract information from the sensed data. In Section~\ref{sec:sensing_and_modeling_context} of this survey we describe how information flows from the physical environment through phones' sensors, and gets processed by the means of machine learning algorithms. We specifically pay attention to challenges in the area of mobile context sensing and modelling. Limitations of mobile hardware, such as modest energy storage capabilities and sensor accuracy are key aspects of the problem. Another one comes from the sensed data, which are often noisy and voluminous. Moreover, a smartphone is a very personal device and as such generates data highly specific to an individual who uses it~\cite{Campbell2008}. Major efforts in the area of \textit{mobile sensing} are geared towards the development of scalable data mining algorithms and  extraction of information from diverse user populations.\mm{changed}
%%Thus, major efforts in the area of mobile sensing are geared towards the development of robust data mining algorithms that scale over a large number of users and properly handle diverse populations. %In Section~\ref{sec:sensing_context} we give an overview of recent work in mobile sensor based context recognition.
%
%% But can we harness mobile phones to predict what is going to happen next? 
%Initial efforts in mobile sensing aimed to extract the context in which a phone is operating. With context recognition a phone becomes a \textit{sense}~\cite{Campbell2012}. While the area is far from being fully explored, recent research is increasingly focusing on providing \textit{cognitive} capabilities to mobile phones. Thus, phones are trained to \textit{predict} future events from current and past sensor data. The ability to anticipate users' location, social encounters or health hazards pushes smartphones further from simple communication devices to irreplaceable personal assistants. While inferring usage context on a smartphone remains difficult due to the sheer amount and quality of highly user-specific data, predicting a future context is even more so. \textit{Anticipatory mobile sensing} is tied with problems such as  identifying properties that allow prediction, obtaining the sufficient amount of past data needed for reliable inference, and, finally, determining whether a prediction is possible at all. Section~\ref{sec:predicting_context} provides an overview of the existing work in predicting user context with smartphones. Certain predictions, such as user's location and activities, are of special significance as they empower phones with the knowledge necessary for impacting user behaviour and comfort. This survey is specifically focused on these aspects of anticipatory mobile sensing.
%
%Finally, predictions made with the help of data gathered through mobile sensing can be used as a basis for intelligent decision making. In Section~\ref{sec:anticipatory_computing} we investigate anticipatory computing systems, applications that rely on past, present and anticipated future in order to make judicious decisions about their actions. Ideas about computing devices that can autonomously adapt their performance over time is not new \cite{Kephart2003}. However, smartphones are potentially a revolutionary platform for anticipatory computing as they bridge the gap between human and computer:
%%First, they fulfill the necessary prerequisites for successful anticipatory reasoning: they are equipped with numerous sensors and can infer and monitor the context, powerful processing hardware allows them to run machine learning algorithms and develop sophisticated models of the future.
%phones are very closely integrated with everyday life of individuals \cite{Katz1998}. Thus, anticipatory computing on mobile phones can be very personal, timely and relevant for the user.
%
%The goal of this survey is to introduce the reader to major contributions in different aspects of the emerging field of \textit{anticipatory mobile computing}, such as mobile sensing, context inference and prediction, and anticipatory computing. Each of these research areas is thoroughly covered in the existing survey literature, such as \cite{Rosen1985,Chen2000,Lane2010,Burbey2012,Lanzi2008}, thus we concentrate on an orthogonal goal and examine the role of each of the stages in the process of designing anticipatory sensing systems. While we provide a thorough overview of the state of the art, our goal is predominantly to get the reader familiar with possible applications of smartphone context prediction, namely, adaptive sensing, feature identification and extraction, and personalized machine learning model development.  Additionally, we discuss key unresolved issues, especially those related to large scale mobile sensing. Finally, while we predominantly concentrate on smartphones as the most ubiquitous representatives of mobile sensing devices, we believe that guidelines presented in this survey should be applicable to emerging, and yet-to-emerge, wearable sensing devices~\cite{GoogleGlass}.

==> tex/02_sensing_context.tex <==
\section{Mobile Sensing and Context Modelling}
\label{sec:sensing_and_modeling_context}

%IN PREVIOUS SURVEY PAPERS:
%+ sensing towards cognitive phones
%- apps: transportation, environment, health, social nets
%+ app stores
%+ scaling
%- programmability 
%+ continuous sensing
%+ crowd-sourcing
%- human behaviour and context modelling 
%- sharing via OSNs
%+ personalized sensing
%- persuasive computing
%- predict social outcomes, group dynamic, personal relationships.

Smartphones have evolved from communication devices to perceptive devices capable of inferring context around them. Mobile phone's ability to infer that its user is jogging~\cite{Miluzzo2008}, commuting to work, sleeping \cite{Lane2011b} or even feeling angry \cite{Rachuri2010}, is enabled by two factors.\mm{maybe add references for each of these activities?} First, modern day smartphones are provisioned with sophisticated \textit{senses} and boast high computational power hardware. A today's phone hosts a touch-screen, GPS, accelerometer, gyroscope, proximity and light sensors, high quality microphones and cameras, in addition to a range of communication interfaces, such as WiFi, Bluetooth, 4G/LTE, and a near-field communication (NFC) interface. Multi-core processors and gigabytes of memory allow smartphones to locally handle a large amount of data coming from these senses and extract meaningful context descriptors. The second key factor that enables phones to infer user behaviour is the increasingly ubiquitous and personal usage of mobile phones. Nowadays, the majority of the world's population owns a mobile phone, and these phones are closely integrated with people's lifestyle. Not only are mobile phones, for a large part of a day, physically present with their owners, phones are also used for highly personal purposes such as organizing meetings, navigation, online social networking and e-commerce.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figs/mobile_sensing_overview_figure.pdf}
    \caption{Mobile sensing: from real-world signals to advanced concepts.}
 	\label{fig:mobile_sensing_challenges}
\end{figure}

Monitoring physical environment and building models that connect raw sensed data to high level concepts represent the core of mobile sensing. In this section we investigate issues related to two key aspects of mobile anticipatory sensing system design: context sensing and modelling. Figure~\ref{fig:mobile_sensing_challenges} depicts a classification of these issues. 
%They broadly fall in two categories: context sensing and context modelling. 
The primary goal of context sensing is to provide an interface between the physical world and a mobile device. Modelling context, on the other hand, concentrates on the collected data manipulation and construction of models that infer interesting events or behaviours from the raw samples. In the area of mobile sensing the two categories are intertwined and incomplete without each other. Yet, historically they have evolved independently. In addition, unique challenges are associated with each of the categories, thus in this section we analyse context sensing and context modelling independently.

\subsection{Sensing Context}
%Wearable computing. 
%Learning patterns of activity using real-time tracking

Computing devices can be truly integrated with the everyday life of individuals only if they are cognisant of their environment. Situations and entities that comprise the environment are collectively termed \textit{context}. Context may have numerous aspects: geographical, physical, social, temporal, organizational, to name a few. Context sensing aims at bridging physical stimuli sensed by device's sensors, also known as modalities, and high level concepts that describe a context. Context sensing is a broad area explored by diverse disciplines, predominantly pervasive computing and robotics. Here we present a brief overview of context sensing for mobile devices. 


\subsubsection{Early Mobile Sensing Systems}

Research in mobile sensing commenced long before smartphones hit the market. Initially, inferring the surrounding context had to rely on purpose-built hardware platforms consisting of independent sensors and a processing device, usually a microcontroller or a laptop. These platforms extended the idea of wearable computing with senses that served to bridge the gap between the physical and digital. 

The Sociometer was one of the first examples of a multi-modal mobile sensing platform \cite{Choudhury2003}. The aim of this project was to automatically and unobtrusively learn social network structures. In order to achieve this design goal, the Sociometer obtained information about human contacts through an infra-red (IR) transceiver and a microphone, all connected to the same micro-controller board. For a social contact to be inferred, first, the IR transceiver had to register the presence of another transceiver ID. However, not all encounters could be classified as social in their nature. Thus, microphone data was processed and if a lively conversation was detected, the Sociometer classified the event as a social contact. The Sociometer project demonstrated how the environment of a mobile device can be inferred with a high accuracy. In addition, it ushered into a new kind of interdisciplinary research where traditional social science concepts are experimentally investigated with the help of mobile sensing.

Extending the idea of the Sociometer, researchers at Intel Research and the University of Washington developed the Mobile Sensing Platform (MSP)~\cite{Choudhury2008}. The MSP was designed as a general purpose sensing device, not only for the recognition of social encounters. Compared to the Sociometer, the MSP includes a wider variety of sensors: a microphone, visible light phototransistor, accelerometer, barometer, temperature and humidity sensor, compass and IR transceiver. The justification for such a large number of sensors came from findings that information gathered by multimodal sensors can offset the ambiguities that arise when a single sensor data is used for inference~\cite{Maurer2006}. Moreover, complementary modalities support the recognition of a wide range of contexts. Thus, the MSP allows inference of human activities such as walking, running, taking stairs, cooking, watching TV, and many others. Consequently, the platform was used as a basis for UbiFit, a body sensing application that infers user's physical well being and through a mobile ambient display encourages individuals to be physically active~\cite{Consolvo2008}. With UbiFit and similar applications mobile sensing advanced from inferring user activities to impacting user behaviour~\cite{Lathia2013}.

%Other platforms \cite{Bharatula2005}

The Sociometer and the MSP are just two examples of wearable multimodal platforms developed for mobile sensing before smartphones took off. Other notable examples include a low-power context sensing platform developed by Bharatula et al.~\cite{Bharatula2005}, and SenSay~\cite{Siewiorek2003}, a system based on on-body sensors that introduces context-awareness to a user's mobile phone. More examples of wearable sensing platforms can be found in a survey by Pantelopoulos and Bourbakis~\cite{Pantelopoulos2010}. Common characteristics of all the above platforms is that they included wearable sensors and a separate data processing device, e.g. a laptop, PDA or micro-controller, and were used for collecting data in well planned experiments. Built for only one purpose -- to collect sensor data -- these systems were significantly different than today's smartphones. Nevertheless, wearable platforms demonstrated that mobile sensing became an irreplaceable tool for monitoring and understanding human behaviour. 

\subsubsection{Obstacles to Mobile Context Sensing}

The need for custom built sensing platform wanes, as today's smartphones avail highly multimodal sensing, and are unobtrusively carried by their owners at all times. However, applications that use smartphone sensing are still subject to standard mobile sensing constraints identified in earlier work on custom sensing platforms ~\cite{Choudhury2003,Choudhury2008}. Resource-constrained challenges have been the focus of the research agenda of many projects, starting from the first mobile sensing prototypes, such as CenceMe~\cite{Miluzzo2008} and BeTelGeuse~\cite{betelgeuse}.

These constraints come from the battery, processing, storage and communication constraints of mobile devices. Energy shortage issues are exacerbated by the design of smartphone sensors as occasionally used features, rather than constantly sampled sensors. A sensing device can reduce its energy consumption either by sampling less often or, in case it hosts multiple sensor types, by preferring low-power sensors to more power hungry ones. Both approaches come with drawbacks of either completely missing to sense important events or sensing them with an insufficient resolution. Here we present two of the most common ways of addressing energy shortage, as well as a few innovative approaches to energy efficiency in mobile sensing.

SociableSense is a mobile application that senses socialization among users \cite{Rachuri2011}. This system operates on commodity phones and achieves energy efficiency by adapting the sampling rate. A linear reward-inaction function is associated with the sensing cycle, and the rate is reduced during ``quite" times, when no interesting events are observed. The approach is very efficient with human interaction inference, since the target events, i.e., conversations, are not sudden and short. On another side of the solution spectrum Energy Efficient Mobile Sensing System (EEMSS) proposed by Wang et al. hierarchically orders sensors with respect to their energy consumption, and activates high-resolution power-hungry sensors, only when low-consumption ones sense an interesting event~\cite{Wang2009}. The management of sensor states and transitions in EEMSS is performed through an XML styled state descriptor that allows the operator to define interesting events and the desired power saving schemes. The Jigsaw sensing engine~\cite{Lu2010} preserves power by triggering power hungry stages of sensing and sensor data processing only when these become necessary for successful tracking of user behaviour. Therefore, Jigsaw discards data sensed by a microphone if the intensity of the samples is below a certain intensity threshold and cannot provide high-level information sought by the application. Similarly, a Markov decision process controls GPS sampling such that the sensing rate is increased when a user moves rapidly, and decreased if the movement is slow. 

Location and movement inference is especially interesting from the adaptive sensing perspective, as inferring the exact coordinates of a person is seldom of direct interest compared to inferring a meaningful description of the location (i.e. a coffee shop, home, university campus). In addition, the GPS sensor is one of the most power hungry sensors on a mobile device, and reducing its sampling rate represents an attractive way to increase energy-efficiency of an application~\cite{SENSLOC}. SensLoc goes beyond the exact coordinate tracking and  recognises important places and paths taken by a user. It relies on a change in the WiFi environment signature in order to detects entrance to or departure from a location. SensLoc further preserves energy by sampling GPS only for path tracking, and only when the phone's accelerometer detects that the user is moving. For trajectory tracking Kj{\ae}rgaard et al. propose adaptive sampling of accelerometer, compass and GPS sensors in order to achieve the most energy efficient trajectory tracking with the given error tolerance~\cite{Kjaergaard2011}. The same work also presents a method for simplified trajectory representation. The identification of the minimal model of a phenomena that we are sensing optimises both sensing energy, but also associated storage and communication overheads.

The inherent structure of the context inference problem can be used to improve sensing efficiency. This is the main idea behind the Acquisitional Context Engine (ACE) proposed in \cite{Nath2012}. Here, Nath develops a speculation-based sensing engine that learns associative rules among contexts, an example of which would be ``when a user state is \textit{driving}, his location is not \textit{at home}". When a context-sensitive application needs to know if a user is is at home or not, it contacts ACE that acts as a middle layer between sensors and the application. ACE initially probes a less energy costly sensor -- accelerometer -- and only if the sensed data does not imply that a user is driving, it turns the GPS on and infers the actual user's location. While demonstrated on simple rules, Nath argues that ACE can be complemented with tools that examine the temporal continuity of context, such as SeeMon \cite{Kang2008} to extract sophisticated rules like ``if a user is \textit{at home} now, he cannot be \textit{in the office} in the next ten minutes".

Cloud computing opens up additional opportunities for improved use of energy resources. Let us consider GPS for example. The location is determined through processing of signals received from Global Navigation Satellite System (GNSS) satellites. Because of a low data rate between a satellite and a device, and complex wireless signal processing, required due to Doppler frequency shifts and weak signal strengths, GPS remains on of the most power hungry sensors in mobile phones. In \cite{Liu2012}, the authors develop CO-GPS -- a system where once it gets detected by a mobile device, raw received signals are uploaded to the cloud for processing, relieving a battery limited device from the burden of computation. CO-GPS consumes up to three orders of magnitude less energy than the conventional GPS system. The drawback is that due to increased communication latitude and longitude determination via CO-GPS lags behind the standard GPS approach. Nevertheless, energy efficient operation through offloading from a mobile phone to a cloud is potentially applicable to other sensing modalities where computation energy is greater than energy needed for cloud uploading. Such modalities most likely  include those where complex signal processing is needed, e.g. sound and video. %However, restrictions on the answer delay and the cost of communication make 


% Compression sensing?

Despite ongoing technological advances mobile phones still have limited processing and data storage capabilities. As mentioned above, remote resources available via online cloud computing can be used to help with data processing. However, the transfer of the high-volume data produced by mobile sensors can be costly, especially if done via a cellular network. 

Balancing local and remote processing was tackled in one of the first smartphone sensing applications, CenceMe~\cite{Miluzzo2008}. This application performs audio and activity classification on the phone, while some other modalities, such as user's location, are classified on a remote server. The distribution of the computation is not performed solely because of the limited computation resources of a smartphone. Distributed computation also allows for aggregation of data from multiple phones, therefore a larger context can be inferred. In CenceMe an ``Am I Hot" classifier of user's social behaviour is developed thanks to distributed, multi-user sensing. Different costs associated with local and remote data processing are examined in~\cite{Rachuri2011}. The split between the two is done on the basis of energy expenditure, data transmission cost, and the computation delay. The decision is made when each of the aspects, available energy, data transfer cost and computation latency, are evaluated through a multi-criteria utility function. Each of the aspects figures in the utility function with a certain weight. An XML-based interface is provided through which one can set simple rules that guide weight adjustment. For example, the energy saving can be given the priority if the battery level is low. 

Certain hardware limitations that hamper mobile sensing, most notably the lack of computing capabilities, are likely to be overcome in near future, Modern cellphones already host multi-core processors and gigabytes of memory. Battery related issues, on the other hand, still represent a significant burden to continuous sensing. Distributed mobile sensing brings new, socially-aware, applications, but with additional challenges of data management. 

%
%\subsubsection{Sensing on Multiple Devices}
%
%Types of mobile sensing: particpatory, opportunitstic.
%
%
%If two or more devices
%have similar sensors, their samples can be merged to
%obtain a possibly more complete view on the
%environment. This has been proposed independently
%in [23],J. Mäntyjärvi, J. Himberg, and P. Huuskonen.
%Collaborative context recognition for handheld
%devices. In First IEEE International Conference on
%Pervasive Computing and Communications
%(PerCom’03), pages 161-168,

\subsection{Modeling Context}
\label{sec:modeling_context}

Raw sensor data, such as those from phone's accelerometer, are seldom of direct interest and machine learning techniques are usually employed to infer higher level concepts, for example, a user's physical activity \cite{Tapia2007}. For the inference to be made, first we need to decide which aspects of the raw sensor data are the most representative of the phenomena we would like to explain. Then, appropriate machine learning techniques are used to build a faithful model of human behaviour and train it with the data gathered so far. Finally, the current context is inferred from the collected data.

\subsubsection{Selecting Useful Modalities and Features from Sensor Data}
\label{sec:select_features}
The first challenge in context modelling is the identification of those modalities of raw data that are the most descriptive of the context. Interdisciplinary efforts and domain knowledge are crucial in this step. For example, if we try to infer user's emotions, the existing work in psychology tells us that emotions are manifested in a person's speech \cite{Bezooijen1983}. Consequently, we can discard irrelevant modalities and concentrate our efforts on processing microphone data.

The next step includes the selection of the appropriate representation for the sensor data. Consider EmotionSense, an experimental psychology research application, which harnesses the fact that a mobile phone microphone can record sufficient information needed for emotion inference \cite{Rachuri2010}. Before the classification, however, raw microphone data has to be transformed to a suitable form. Distinctive properties extracted from the data are called \textit{features}. The EmotionSense authors built its speech recognition models on Perceptual Linear Predictive (PLP) coefficients, a well established approach to speech analysis \cite{Hermansky1990}. An alternative, but less sophisticated means of microphone data manipulation that has proven successful in mobile sensing is the Discrete Fourier Transform (DFT) \cite{Miluzzo2008}. The majority of speech energy is found in a relatively narrow band from 250 Hz to 600 Hz, thus the investigation of DFT coefficient means and variations can help identify speech in an audio trace. Finally, Mel-Frequency Cepstral Coefficients (MFCC) are another commonly used feature for speech recognition \cite{Lu2009,Miluzzo2010,Chon2012}.

\begin{table}[htb]
%\figsp
\begin{center}
\begin{scriptsize}
\begin{tabular}{|c|l|}
\hline
\textbf{Domain} & \textbf{Characteristic Features} \\
\hline
\hline
Speech recognition & 
\begin{tabular}[l]{@{}l@{}} -- Sound spectral entropy, RMS, zero crossing rate, low energy frame rate,\\
 spectral flux, spectral rolloff, bandwidth, phase deviation\\
\cite{Lu2009,Lane2011b}\\
-- Mel-Frequency Cepstral Coefficients (MFCCs)\\
\cite{Lu2009,Miluzzo2010,Chon2012}\\
\cite{Lu2010,Lu2012}\\
-- Teager Energy Operator (TEO), pitch range, jitter and standard deviation,\\
spectral centroid, speaking rate, high frequency ratio\\
\cite{Lu2012,Lu2010}\\
-- Running average of amplitude, sum of absolute differences\\
\cite{Krause2006}\\
-- Perceptual linear predictive (PCP) coefficients\\
\cite{Rachuri2010}\\
-- Mean and standard deviation of DFT power\\
\cite{Miluzzo2008}


%MFCC, Teager Energy Operator (TEO), Pitch range, jitter and stdev, Spectral centroid, speaking rate, high frequency ratio Lu2012, Lu2010 (without TEO)
%Running average of amplitude, SAD KRause2006
%Sound: Spectral entropy, RMS, zero crossing rate, low energy frame rate,spectral flux, spectral rolloff, bandwidth, phase deviation Lu2009, Lane2011b
%Speech: auto correlation, spectral entropy Choudhury2003
%HMM + MFCC Chon2012
%Music: GMM + MFCC Chon2012
%MFCC - Miluzzo2010
%Mean+ STDEV of DFT power Miluzzo2008
%Perceptual linear predictive (PLP) coefficients  Rachuri2010

\end{tabular}\\
\hline
Activity classification & 
\begin{tabular}[l]{@{}l@{}}-- Accelerometer FFT principal component analysis (PCA)\\
\cite{Krause2006}\\
-- Accelerometer intensity/energy/mean\\
\cite{Eston1998,Lu2010,Rabbi2011,Abdullah2012}\\
-- Accelerometer variance\\
\cite{Miluzzo2008,Lu2010,Rabbi2011,Aharony2011}\\
-- Accelerometer peaks/mean crossing rate\\
\cite{Miluzzo2008,Lu2010}\\
-- Accelerometer spectral features
\cite{Lu2009,Lu2010,Lane2011b,Rabbi2011}\\
-- Accelerometer correlations\\
\cite{Abdullah2012}\\
-- Accelerometer frequency domain entropy\\
\cite{Abdullah2012}\\
-- Barometric pressure\\
\cite{Rabbi2011}

\end{tabular}\\
\hline

Location & 
\begin{tabular}[l]{@{}l@{}}
-- Days on which any cell tower was contacted, \\
days on which a specific tower is contacted, \\
contact duration, events during work/home hours\\
\cite{Isaacman2011}\\
-- Tanimoto Coefficient of WiFi fingerprints \\
\cite{Chon2012}\\
-- Eigenbehaviors - vectors of time-place pairs\\
\cite{Eagle2009b}\\
-- Hour of day, latitude, longitude, altitude, social ties\\
\cite{DeDomenico2012}\\
\end{tabular}\\
\hline
Object recognition & \begin{tabular}[l]{@{}l@{}}-- GIST features\\
\cite{Chon2012}
\end{tabular}\\
\hline
Gestures & \begin{tabular}[l]{@{}l@{}}-- Mean, max, min, median, amplitude, and\\
high pass filtered values of acc. intensity and jerk;\\
spectral features; screen touch location, slope, speed,\\
strokes number, length, slope and location\\
\cite{Coutrix2012}\\
\end{tabular}\\
\hline
Physiological state & \begin{tabular}[l]{@{}l@{}}-- Galvanic skin response, heat flux,\\
skin thermometer running average and sum of absolute differences\\
\cite{Krause2006}\\
\end{tabular}\\
\hline
Thoughts & \begin{tabular}[l]{@{}l@{}}-- Bandpass filtered neural signal from EEG\\
\cite{Campbell2010}\\
\end{tabular}\\
\hline
Call prediction & \begin{tabular}[l]{@{}l@{}}--  Call arrival and inter-departure time, calling reciprocity\\  \cite{Phithakkitnukoon2011}\\
\end{tabular}\\
\hline
Interruptibility & \begin{tabular}[l]{@{}l@{}}-- User typing, moving, clicking, application focus, app. activity, \\
gaze, time of day, day of week, calendar, acoustic energy, WiFi environment,\\
\cite{Horvitz2003}\\
-- Mean, energy, entropy and correlation of accelerometer data\\
\cite{Ho2005}
\end{tabular}\\
\hline
\end{tabular}
\end{scriptsize}
\caption{}%Summary of machine learning techniques.}
\label{tab:features}
\end{center}
\end{table}

%
%Depression in Bipolar disorder: self-reported mood rating Moore200?
%
%Social contacts: work or not, time of day, Bluetooth environment Ealgle2006
%
%The following are done via regression:
%
%Health state: phone calls, SMSs, communication diversity, BT rpoximity, WLAN APs distribution, late-night, early-morning communication Madan2011.
%
%Political opinion change: time, political opinion, type of interaction, amount of interaction, self-reported relationship. Madan2011
%
%Thoughts:
%bandpassed filtered neural signal from EEG Campbell2010
%%
%Physiology: galvanic skin response, heat flux and skin thermometer running average and sum of absolute differences. Krause2006

%Gesture recognition:accelereometer and acc. jerk mean, max, min, median, amplitude, variance , also high-pass filitered values. Spectral analysis: important frequencies;
%touch location, touch slope, touch speed, num strokes, stroke lengths and locations, slopes <-min max mean median,. amplitude of all the above Coutrix2012
%
%Call prediction: call arrival time, interdeparture time, calling reciprocity Phithakkitnukoon2011
%Interruptibility: whether a user is typing, moving or clicking with the mouse, current focus, application used, application activity, gaze, windows switching, opened windows, time of day, day of the week, if a meeting exists, acoustic energy, user location as determined with WiFi Horvitz2003
%mean, energy, entropy and correlation of accelerometer data Ho2005

%Activity Accelerometer FFT + PCA Krause2006; accelerometer intensity Eston1998; accelerometer variance Aharony2011
%Energy, mean, variance and spectral features of the accelerometer + variance and signed change in pressure over various time windows for barometric pressure data Rabbi2011
%Mean, variance, mean crossing rate, spectrum features of accelerometer Lu2010
%Mean, energy, freq-domain entropy, correlation of accelerometer Abdullah2012
%Mean, STDEV, num of peaks of acceleremeter Miluzzo2008
%
%Voice: Stress: MFCC, Teager Energy Operator (TEO), Pitch range, jitter and stdev, Spectral centroid, speaking rate, high frequency ratio Lu2012, Lu2010 (without TEO)
%Running average of amplitude, SAD KRause2006
%Sound: Spectral entropy, RMS, zero crossing rate, low energy frame rate,spectral flux, spectral rolloff, bandwidth, phase deviation Lu2009, Lane2011b
%Speech: auto correlation, spectral entropy Choudhury2003
%HMM + MFCC Chon2012
%Music: GMM + MFCC Chon2012
%MFCC - Miluzzo2010
%Mean+ STDEV of DFT power Miluzzo2008
%Perceptual linear predictive (PLP) coefficients  Rachuri2010
%
%Location (with BT or WiFi): eigenbehaviors - vectors of time-location pairs Eagle2009
%Tanimoto Coefficient of WiFi fingerprints Chon2012
%Location with cell towers: days on which any cell tower was contacted, days on which a specific tower is contacted, contact duration, events during work and home hours: Isaacman2011
%
%Object recognition: GIST features (FIND REF!) Chon2012

The above discussion shows that numerous features can be extracted from a single modality. In many domains, however, certain feature types have crystallized out as the most informative. Table~\ref{tab:features} lists the most commonly observed features and the domains in which they are used. The table is not meant to be a comprehensive survey of feature extraction, but should point out that even with a small number of sensors there can be hundreds of possible features all of which may or may not contribute to context inference~\cite{Choudhury2008}. To tackle the problem of feature selection one possibility is to employ computationally inexpensive mathematical transformation known as the Principle Component Analysis (PCA)~\cite{Pearson1901}, as demonstrated in~\cite{Krause2006}. After the PCA is performed we are left with a set of most promising features that impact the target variable the most, i.e., in this case the aspect that we want to infer. However, different classifiers might give different results even with the same features. Wrapping is used as a more accurate, albeit more computationally complex, alternative to PCA~\cite{Kohavi1997}. In this procedure, based on the collected data, a classifier is built with each of the subsets of features. A part of the data is left out during the training phase and is used to evaluate the classifiers. An example of wrapping based feature selection can be found in the human interruption study by Fogarty et al.~\cite{Fogarty2005}. A boosting-based technique for ranking features according to their contribution towards context recognition has been proposed by Lester et al.~\cite{Lester2005}. Their approach iteratively trains an ensemble of weak binary classifiers constrained to use a single feature each. At the end of the training we are left with not only the ranking of features, but also with the weights that indicate how important each of the features is for the final classification. Interestingly, the same classifier, used in different environments, may require different features for successful classification. For example, Lu et al. find that a standard speech classification attribute MFCC does not perform well outdoors while more noise tolerant features, such as high frequency energy ratio and frequency centroid become more discriminative in this setting~\cite{Lu2012}.

Modality and feature selection impact the rest of the context inference; a careful consideration at this stage of the process can help improve classification accuracy or reduce the computational complexity of the learning process. With an increasing number of sensors and a growing interest in a variety of context domains, identifying and quantifying the strength of a link between a domain and a modality or a feature emerges as an important research direction in mobile sensing.
%Unfortunately, in many domains we still cannot answer a question of whether a link between a concept and a modality or a feature can be established.\mm{This comment might sound a bit vague - perhaps add more details}


\subsubsection{Classification Methods}
\label{sec:classification_methods}
The construction of models is a crucial part of the design of context inference systems. A plethora of machine learning techniques at our disposal can be used to transfer distilled sensor data into mathematical representations of user behaviour. In this survey we concentrate on a small subset of machine learning techniques that have been successfully applied to mobile sensing problems, and we refer an interested reader to machine learning texts such as, for example,~\cite{Bishop2006,elementsstatisticallearning2009,RG11:first,Bar12:Bayesian}.

We examine how context inference models are built in case of StressSense, mobile phone application that analyses speech data collected via a built-in microphone and identifies if a user is under stress \cite{Lu2012}. The first step in StressSense is sound and speech detection. The application assumes that sound is present if high audio level is present in at least 50 out of 1000 samples taken within a half a second period. In such a case, StressSense divides the audio signal into frames and for each of the frames calculates its zero crossing rate (ZCR) and root mean square (RMS) of the sound. These features correspond to sound pitch and energy. A tree-based classifier that decides between speech and non-speech frames is built with ZCR and RMS as attributes. Further, thresholds on ZCR and spectral entropy are used to discern between voiced and unvoiced frames of human speech. Finally, Gaussian Mixture Models (GMMs) are built for the two target classes -- stressed speech and neutral speech. Pitch, Teager Energy Operator (TEO) and Mel-Frequency Cepstral Coefficient (MFCC) based features of each voiced frame are used for user stress inference.\vp{Added example, consistent with the previous subsection that also has an example.}

The variety of classification methods and data features opens up wide opportunities for novel context inference methods. Yet, the structure of the problem at hand often hints towards classification approaches that we system designers should consider. In Table~\ref{tab:learners} we list mobile sensing challenges and the corresponding machine learning techniques that have been proved to work well in practice. 

%Thus, phenomena that exhibit smooth transitions among states are naturally modelled by Markov chains. 
%Daily movement of a person often includes visits to the same set of places, e.g. home, work, school, in a well defined order. Time series analysis proves to be a suitable technique in this domain \cite{Scellato2011,DeDomenico2012}. 
However, irrespective of the domain, in machine learning, data is king. A simple classifier built upon a large amount of data usually outperforms even the most complex classifier trained with insufficient information. Moreover, the amount of training data at our disposal determines the optimal classifier. Therefore, Naive Bayesian classifier usually performs well even with little data, as each feature can be independently estimated as an one dimensional distribution. This helps alleviate problems stemming from the curse of dimensionality, i.e., the need for data sets that scale exponentially with the number of features. More elaborate classification algorithms such as support vector machines (SVMs)~\cite{Cristianini2000} require more training data. Further, Forman and Cohen show that classifier performance depends on the distribution of classes in the training data set. This impacts both model selection as well as  feature selection, as different combinations of features and classifiers work best for different training data sets~\cite{Forman2004}.

\begin{table}[htb]
%\figsp
\begin{center}
\begin{scriptsize}
\begin{tabular}{|c|l|}
\hline
\textbf{Domain} & \textbf{Machine learning technique} \\
\hline
\hline
Speech recognition & 
\begin{tabular}[l]{@{}l@{}} -- Hidden Markov Model (HMM)\\ \cite{Chon2012,Choudhury2003}\\-- Threshold based learning \cite{Wang2009}\\-- Gaussian Mixture Model (GMM) \cite{Rachuri2010,Lu2012}\end{tabular}\\
%Complex: a function of locally relevant content, language and supporting infrastructure & Yes 
\hline
Activity classification & 
\begin{tabular}[l]{@{}l@{}}-- Boosted ensemble of weak learners\\ \cite{Consolvo2008,Abdullah2012}\\
-- Boosting \& HMM for smoothing \cite{Lester2005}\\-- Tree based learner \\  \cite{Tapia2007,Abdullah2012}\\-- Bayesian Networks~\cite{Krause2006}\end{tabular}\\
\hline
Location determination (with GPS) & 
\begin{tabular}[l]{@{}l@{}}-- Markov chain\cite{Ashbrook2003}\\
-- Non-linear time series \\ \cite{Scellato2011,DeDomenico2012}\end{tabular}\\
\hline
Location (with BT or WiFi) & \begin{tabular}[l]{@{}l@{}} -- Bayesian network\\
\cite{Eagle2006,Eagle2009a}\end{tabular}\\
\hline
Location (with ambient sensors) & -- Nearest neighbour \cite{Maurer2006}\\
\hline
Scene classification & -- K-means clustering \cite{Chon2012}\\
\hline
Object recognition & \begin{tabular}[l]{@{}l@{}}-- Support vector machine \cite{Chon2012}\\
-- Boosting \& tree-stump \cite{Wang2012}\end{tabular}\\
\hline
Place categorization & -- Labelled LDA~\cite{Chon2012}\\
\hline
Call prediction & -- Naive Bayesian \cite{Phithakkitnukoon2011}\\
\hline
Interruptibility & \begin{tabular}[l]{@{}l@{}}-- Bayesian Network \\ \cite{Horvitz2003,Fogarty2005}\\ -- Tree based learner \cite{Fogarty2005}\\
-- Naive Bayes~\cite{Hofte2007}\end{tabular}\\
\hline
\end{tabular}
\end{scriptsize}
\caption{}%Summary of machine learning techniques.}
\label{tab:learners}
\end{center}
\end{table}


%Data structure? 
%
%Tradeoff between accuracy and complexity.
%
%
%Speech recognition - HMM~\cite{Chon2012,Choudhury2003}, threshold based\cite{Wang2009}, Gaussian Mixture Model \cite{Rachuri2010}
%
%Activity classification - tree based, Boosted ensemble~\cite{Abdulah2012}, Boosted decision stump~\cite{Consolvo2008}, Bayesian Networks~\cite{Krause2006}, Boosting + HMM for smoothing \cite{Lester2005}, thereshold based\cite{Wang2009}, decision tree \cite{Tapia2007}
%
%Location determination (GPS) - Markov Chain~\cite{Ashbrook2003}, Non linear time series~\cite{NextPlace}, \cite{DeDomenico}
%
%Location determination (BT or WiFi fingerprinting) - Bayesian Net~\cite{Eagle2006}, \cite{Eagle2009}
%
%Location determination (light, motion, audio, temperature) - nearest neighbor\cite{Maurer2006}
%
%Scene classificatioon - k-means clustering \cite{Chon2012}
%
%Object recognition - support vector machine \cite{Chon2012}, AdaBoost+TreeStump\cite{Wang2012}
%
%Place categorization - Labelled LDA~\cite{Chon2012}
%
%Human interruptibility - Bayesian Network~\cite{Horvitz2003}, Naive Bayes~\cite{Hofte2007}.
%
%Call prediction - Naive Bayesian \cite{Phithakkitnukoon2011}
%
%
%CHECK KRAUSE
%
%Thus, extracting Mel-Frequency Cepstral Coefficients and employing Gaussian Mixture Models has crystallized out as the most promising approach to sound classification~\cite{Lu2009, Rachuri2010, Miluzzo2010, Chon2012}, while tree-based classification or boosted ensemble of weak classifiers successfully tackle physical activity classification from accelerometer readings~\cite{Lester2005, Tapia2007, Miluzzo2008, Rabbi2011}.  

\subsubsection{Handling Large-Scale Inference}
\label{sec:large_scale}

Mobile sensing is moving from modelling behaviour of a small group of test users to observations of large populations. A recent trend is for mobile sensing applications to be distributed through commercial app stores such as iTunes and Google Play~\cite{Rachuri2010,Miluzzo2008}. Consequently, researchers sacrifice the comfort of being able to physically interact with study subject for the ability to gather larger, more diverse data. Novel challenges with respect to sensing application distribution, data processing and scalable machine learning have emerged. Data diversity calls for more complex classification: walking performed by an eighty year old person will yield significantly different accelerometer readings than when the same activity is performed by a twenty year old. Clearly, activity classification needs to be less general, but does that imply a personal classifier for each user? 

In~\cite{Lane2011a} Lane et al. propose community similarity networks (CSNs) that connect users who exhibit similar behaviour. User alikeness is calculated on the basis of their physical characteristics, their lifestyle and from the similarity between their smartphone-sensed data. For each of these three layers in the CSN, a separate Boosting-based classifier is trained for any individual user. However, a single-layer classifier is trained on the data coming from not only the host user, but also from all the other users who show strong similarity on that CSN layer. In this way the CSN approach tackles the shortage of labelled data for the construction of personalized models, a common issue in mobile sensing.

Besides increased user diversity, modern mobile sensing applications often put an emphasis on long-term observations. In their ``social fMRI'' study Aharony et al. gather over 25 sensing modalities continuously for more than a year from about 130 participants \cite{Aharony2011}. Machine learning algorithms need explicit labelling of the high level concepts that are extracted from sensor readings. However, with highly multi-modal sensing integrated with everyday life, querying users to provide descriptions of their activities becomes an intrusive procedure that may annoy them. Instead, a semi-supervised learning technique called \textit{co-training} is used to establish a bond between those sensor readings for which labels exist, and those for which only sensor data are present~\cite{Zhu2009}. Co-training develops two classifiers that provide complementary information about the training set. After the training on the labelled data, the classifiers are iteratively run to assign labels to the unlabelled portion of the data. In the mobile realm, unlabelled data representing an activity of one user could be similar to labelled data of the same activity performed by another user. In this case, labels can propagate through the similarity network of users~\cite{Abdullah2012}. 

In addition to a larger user base and an increased amount of gathered data, mobile sensing is further challenged by a growing number of devices used for context-aware applications. We increasingly observe \textit{ecosystems of devices}, where multiple devices work together towards improved context sensing. Fitbit, for example, markets a range of wearable devices that track user metrics such as activity, sleep patterns, and weight \cite{Fitbit}. As the popularity of these devices grows we can expect that a single user will carry a number of context sensing devices. Darwin Phones project tackles distributed context inference where multiple phones collaborate on sensing the same event \cite{Miluzzo2010}. First, via a cloud infrastructure, phones exchange locally developed models of the target phenomenon. Later, when the same event is sensed by different phones, inference information from each of the phones is pulled together so that the most confident description of the event is selected.

\subsection{Beyond Direct Observations}
Mobile sensing is not limited to inferring directly observable physical activities. Social signal processing (SSP) has emerged as a new research domain where behavioural cues such as gestures, conversations, facial expressions, and others are inferred and interpreted by means of machine learning and artificial intelligence tools~\cite{Pentland08:honest,Vinciarelli2009}. These cues, termed social signals, can be automatically analysed to understand, but also to mimic natural human behaviour \cite{Vinciarelli2012}. Analysing and synthesising behaviour solely with modalities available to machines, usually cameras and microphones, is a very hard task. Restriction to a phone renders this problem even harder to solve, due to increased noise and rapid context change that stems from user mobility and phone placement. Still, sophisticated states of individual and group psyche are increasingly in the focus of recent research on behaviour sampling. For example, EmotionSense, discussed in Section \ref{sec:select_features}, relates the way words are uttered during human speech with emotions the person experiences at the moment~\cite{Rachuri2010}. Likewise, StressSense, that we touched upon in Section \ref{sec:classification_methods}, uses mobile phone's microphone to measure user's stress levels~\cite{Lu2012}.Thought inference is the subject of NeuroPhone, a system that integrates brain signal reading with a mobile phone~\cite{Campbell2010}. The main motivation for NeuroPhone are novel hands-free interfaces, but one can envision applications that build complex intelligence by merging user's thoughts with phone's sensing and computational resources.


With a wealth of sensors on a mobile phone, information about mood can be correlated with user's location or activity, and used to identify novel psychological relationships among these concepts. Indeed, smartphones have a potential to completely revolutionize the way experimental social science research is done, as in situ examination of user's behaviour can be performed via a phone \cite{Miller2012}. In \cite{deMontjoye2013} the authors analyse mobile phone logs and establish relationships between the descriptors of users' calls, contacts and movement, and personality traits. Records of the way a user interacts with a touchscreen, or the way he moves a phone around can help identify hard-to-monitor affective behaviour~\cite{Coutrix2012}. Examining Bluetooth encounters among phones carried by office workers can help measure sociability and improve productivity~\cite{Rachuri2011}. Mobile phones can be used to uncover a wealth of information about us: from socio-economic factors \cite{Lathia2012,Martinez2012}, over our mental and physical health \cite{Rabbi2011,MCMFP12:sensing} to our thoughts~\cite{Campbell2010}. We believe that mobile sensing will also have an increasing role in the emerging area of computational social science~\cite{Lazer2009}.



==> tex/03_predicting_context.tex <==
\section{Anticipatory Sensing}
\label{sec:predicting_context}

Mobile sensing applications do not end at the point where a strong relationship between events we are interested in and the corresponding smartphone sensor data is established. Information collected during the inference phase can also serve as a basis for prediction of future events. Powerful machine learning algorithms and fine-grain sensor data represent a foundation for emerging applications that deliver accurate personalized predictions of future events. In a transition that Campbell and Choudhury call \textit{from smart to cognitive phones}, we can expect smartphones to become proactive personal assistants that anticipate and react upon our actions based on patterns learnt from our daily life~\cite{Campbell2012}. Such smartphones have the potential to co-exist in a symbiosis with their users and narrow the mismatch between the technology and humanity. They will allow for users' movement and action anticipation; they will know when to attract user's attention and when to stay silent; and they will warn their owners of important events or potential hazards. Finally, predictive smartphones will close the loop providing valuable feedback and information to users. Examples include applications for behaviour change~\cite{Lathia2013}.
%With such a personal assistant, people will no longer forget to pack books in the morning of a day that they will pass by a library, or be unprepared for a sudden job interview phone call.

\subsection{Improving Human-Computer Interaction Through Anticipatory Sensing}
\label{sec:improvingHCI}

Context predictions enabled through mobile sensing can serve as a basis for device's adaptation to its owners' lifestyle. Mobile phones are used in a highly personalized context and a need arises for their customized interaction with individual users. Basic personalization can came from explicit rules that a user sets, such as the assignment of speed dial numbers or ringer sounds. However, phone's ability to predict user behaviour allows seamless integration with user's daily routine. An example of a mobile phone system that anticipates, and adapts to user behaviour is the call predictor developed in~\cite{Phithakkitnukoon2011}. The authors devise an outgoing call predictor termed ``Incoming Call Forecast" and an outgoing call predictor, which they refer to as an ``Intelligent Address Book". The former can help people optimize their daily schedules, while the latter, by giving higher preference to those contacts that are more likely to be called, improves navigation through user's address book. For both purposes a probabilistic model that captures the caller's behaviour, the callee's behaviour, reciprocity between the two, and the behaviour trends is built. Calling times often exhibit daily periodic patterns, thus time-of-day and call inter-arrival times prove to be reliable features for building such a prediction model. 

In his 1991 manifesto of ubiquitous computing Weiser advocates pervasive technology that coexists unobtrusively with its users \cite{Weiser1991}. This ``calm technology" is not our current reality, and indeed we get an abundance of notifications from an increasing number of devices we own. Thus, we receive irrelevant instant messages while working on an important project, a phone may sound an embarrassing ``out of battery" tone in the middle of a meeting, and a software update pop-up may show up while we are just temporarily connected to a hot spot in a coffee shop. 

\textit{Attentive user interfaces} manage user attention so that the technology works in symbiosis with, rather than against user's interruptibility. Frameworks for inferring user's availability had been developed before the smartphones era. In~\cite{Horvitz2003}, relying on an external camera and a microphone, along with the information about user's desktop computer usage, the authors develop a framework for inferring user's workload in an office setting. A Bayesian network is then constructed in which variables such as the presence of voice, user's head position and gaze, currently opened applications on a user's PC, are connected with the probability distribution of interruptibility. In another early work Fogarty et al. investigate which sensors should be constructed in order to efficiently infer interruptibility \cite{Fogarty2005}. They embrace a \textit{Wizard of Oz} technique, where human subjects simulate sensors by manually coding information from audio and video recordings. Despite the approach that allows examination of sensors that are yet to be implemented in reality, the authors find that simple sensors often provide enough hints to discern if a user is interruptible or not. Thus, detection of speech in the room remains the most powerful indicator of a non-interruptible state.

The above interruption studies are of great importance in the field of experience sampling.  Experience sampling is a common research technique in psychology~\cite{Hektner2006} where users are asked to provide information about their current experiences in real time. Mobile devices revolutionized this research field, as they enable in-situ probing of users' daily lives. Specialized smartphone frameworks for experience sampling have been developed recently \cite{Froehlich2007,Rachuri2011,Ramanathan2012}. Still, assessing interruptibility remains an important problem, and, beyond isolated attempts, the area remains largely unexplored. 
One of the most representative papers in this area is~\cite{Ho2005} by 
Ho and Intille: in this work the authors
show how an accelerometer can be used to infer activity transitions, period when, the authors argue, a user is more susceptible to interruption~\cite{Ho2005}. Accelerometer movement is just one of many modalities that modern smartphones can sense, and interruptibility prediction for social science experiments remains to be fully explored.


%In~\cite{Horvitz2003}, the authors develop a framework for inferring user's workload in an office setting. Done before the smartphones era, in order to infer interruptibility the proposed framework utilizes an external camera and a microphone, along with the information about user's desktop computer usage. The authors define the \textit{cost of interruption}, a metric that indicates how much a user is willing to pay to avoid an annoying event/notification of a certain type in a certain state. In every moment a sum of the probability that a user is in a specific state\mm{this part is unclear - why do you consider a sum of probability here? which kind of probability we are talking about here?} multiplied by the cost of interruption at that state represents the expected cost of interruption. A Bayesian network is then constructed in which variables such as the presence of voice, user's head position and gaze, currently opened applications on a user's PC, are connected with the probability distribution of interruptibility. Besides the current state, the method also forecasts times when a low, medium, or high state of interruptibility will be reached. In addition, the model seeks to find lingering times in each of the states. For example, it can predict time when a low interruptibility state in which a user will stay for at least five minutes is going to be reached.\mm{maybe this part should be shortened. We need to make clear that this work is not about anticipatory mobile sensing. Perhaps we should also say why this is relevant for mobile sensing}

%In another early work Fogarty et al. investigate which sensors should be constructed in order to efficiently infer interruptibility \cite{Fogarty2005}. They embrace a \textit{Wizard of Oz} technique, where human subjects simulate sensors by manually coding information from audio and video recordings. Despite the approach that allows examination of sensors that are yet to be implemented in reality, the authors find that simple sensors often provide enough hints to discern if a user is interruptible or not. Thus, detection of speech in the room remains the most powerful indicator of a non-interruptible state. The authors employ Naive Bayesian and tree-based machine learning algorithms, along with correlation-based and wrapping feature selection methods. In all cases simple sensors such as a microphone, mouse and keyboard activity, and telephone engagement sensor, provide sufficient information in order to infer interruptibility. Fogarty et al. also examine how interruptibility models evolve with the amount of data and the number of users under study \cite{Fogarty2004}. The analysis shows that the model needs little bootstrapping data before it starts producing high accuracy inferences. Moreover, training data from another user can substantially improve inference when the original user's data is not yet available. Generalizability of the findings, however, should be treated with caution. Two office workers considered in the study might have similar attention patterns, but people who work in different environments might not. \mm{also this is not really about mobile sensing: it should be shortened in my opinion. We also need to make clear why this is relevant for the prediction of context}

%Fogarty et al. point out to an important property of interruption: it is not an one off process, but a negotiated process where the interrupter probes and backs off if the subject is not interruptible at the moment. Kapoor and Horvitz evaluate how annoying different probing strategies are for a subject under study \cite{Kapoor2008}. Decision-theoretic strategies that construct a predictive model about user's internal state\mm{what do you mean by "user internal state" here? This should be clarified}, compute the expected value of information and weight the costs and benefits of probing act more in synchrony with the actual user behaviour than strategies that generate probes for situations associated with the most uncertainty, or at random times. Finally, Kapoor and Horvitz point out that a successful strategy has to follow changes in context over time and adapt to them. They develop one such strategy that not only learns, but forgets concepts that do not get reinforced over time. Their approach is based on decision-theoretic active learning. More details can be found in~\cite{Kapoor2007}. Context ``drift'' has been observed in other human behaviour classification problems as well. In the call prediction system we mentioned earlier, the authors note that recent trends in calling behaviour tend to be more indicative of the future calls than the whole history of caller/callee's behaviour~\cite{Phithakkitnukoon2011}. %pointing out an important problem in behavior prediction - how to tackle concept drifts and incorporate forgetting in online machine learning.


%
%- Horvitz2003: introduce the cost of interrupting a user in state A with an event D as willingness to pay to avoid the interruption. In every moment we can compute the expected cost of interruption by summing up the probability that the user is in a state A multiplied by the cost of interruption at the state A with the event D.
%
%- Horvitz2004: only one state in BusyBody. Employed Bayesian but switched to Gaussian Process classification due to easier computation of the value of information
%
%- Kapoor 2008: comparison of different experience sampling methods. Decision theoretic dynamic probe probes when the expected value of the information gathered is high.
%
%- Ho 2005: trigger messages when a user is shifting between activities
%
%
%- Fogarty 2004: "focus should not be on reducing interruptions, but making them more efficient", models should adapt to a type of user. Investigation of how much data is needed to build a model. How a model built for one type of personality works for another one.
%
%- Hofte2007: which parameters determine user availability and which parameters are users willing to share.
%- Horwitz 2004: notification throttling
%- Horwitz 2003: importance of personalized models
%
%- Fogarty 2005: Interruption is not a one off process. It is a negotiated process. We probe the interruption and back of if the person is not interruptible. 


\subsection{Predicting User Mobility and Behaviour}

Historically, prediction of mobile phone users' movement patterns was tied with system optimizations. Anticipation of surges in the density of subscribers in a cellular network was proposed for dynamic resource reservation and prioritized call handoff~\cite{Soh2003}. Yet, as data collected by a phone gets more personal, the opportunity for novel user-centric anticipatory applications increases. 

User movement was initially explored in the indoor context. With respect to such applications, existing systems usually rely on the use of sensors embedded in the buildings. A significant example of such systems is MavHome: the authors proposes a smart home which adjusts indoor light and heating according to predicted movement of house inhabitants~\cite{Cook2003}. 

Instead, most of the current projects based on mobile phones focus on the prediction of users' movement at a city scale. The first projects in this area focussed on the extraction of significant places for the users~\cite{Ashbrook2003,hightower2005}. Proliferation of location-based services such as Foursquare \cite{Foursquare} raised the interest in user whereabouts prediction from the commercial side. For example, targeted ads can be disseminated to users who are expected to devote a certain amount of their time to eating out or entertainment. Thus, the NextPlace project aims to predict not only user's future location, but also the time of arrival and the interval of time spent at that location \cite{Scellato2011}. The authors rely on a non-linear time series analysis for such a prediction. More recently, Horvitz and Krumm devise a method for predicting a user's destination and suggesting the optimal diversion should the user want to interrupt his/her current trip in order to, for example, take a coffee break \cite{Horvitz2012}. Noulas et al. investigate next check-in prediction in the Foursquare network \cite{Noulas2012}. They show that a supervised learning approach that takes into account multiple features, such as the history of visited venues, their overall popularity, observed transitions between place categories, and other features, need to be jointly considered for a successful prediction. These systems involve the prediction and classification of locations of multiple users performed locally on the device or in the back-end.  For instance, intertwined movement patterns of multiple users in an urban scenario are exploited in the work by McNamara et al.~\cite{McNamara2008}. The authors propose a system for sharing media files among urban commuters who are expected to traverse the same route. A probabilistic reasoning framework for context-aware decisions for supporting drivers have been presented in~\cite{Ziebart08}. The framework is built upon reinforcement learning algorithms based on the analysis of the preferred routes of the drivers. The evaluation of this work is performed on the collection of mobility traces of 25 taxi drivers over 3 months.

Mobile sensing for location prediction does not need to be limited to GPS coordinate tracking. Supplementing and substituting GPS information with phone's accelerometer readings has been proposed for improving energy efficiency of location prediction \cite{Zhuang2010,BenAbdesslem2009}. Moreover, additional context can increase the accuracy of prediction. Thus, SurroundSense utilizes audio and video sensors to assign an audio-visual fingerprint to a location \cite{Azizyan2009}. 

Research on mobility prediction was additionally boosted by large sets of multimodal data that have been collected and made publicly available by companies and academic institutions. For example, the MIT Reality Mining~\cite{Eagle2006} project released a collection of traces from one hundred subjects monitored over a period of nine months. Each phone was preloaded with an application that logged incoming and outgoing calls, Bluetooth devices in proximity, cell tower IDs, application usage, and phone charging status. Similarly, the Nokia Mobile Data Challenge (MDC) data set was collected from around 200 individuals over more than a year \cite{Laurila2012}. The logs contain information related to GPS, WiFi, Bluetooth and accelerometer traces, but also call and SMS logs, multimedia and application usage. The above data sets served as a proving ground for a number of approaches towards location prediction. In~\cite{Eagle2009a} Eagle et al. demonstrate the potential of existing community detection methodologies to identify significant locations based on the network generated by tower transitions. The authors use a dynamic Bayesian network of places, conditioned on towers, and evaluate the prediction on the Reality Mining data set. De Domenico et al. exploit movement correlation and social ties for location anticipation~\cite{DeDomenico2012}.  Relying on nonlinear time series analysis of movement traces from friends or people with correlated mobility patterns, the authors demonstrate improved accuracy of prediction on the MDC data set. Interdependence of friendships and mobility in a location-based social network was also analyzed in~\cite{Cho2011}. Finally, besides its expansion to cover larger user groups, the field of mobility prediction is also advancing towards broader prediction time horizons. Recently, it has been shown that, by extracting recurring patterns in human mobility, predictions can go even months into the future~\cite{Sadilek2012}.


Multimodal traces also enabled activity or behaviour prediction. Human activity recognition has been an active subject of research in the past years: various approaches have been presented in the literature, based for example on accelerometer~\cite{Choudhury2008,Tapia2007}, state-change sensors \cite{Tapia2004} or a system of RFIDs \cite{Wyatt2005}. 

The exploitation of location information together with other sensor data is an active and very promising research area. In a series of seminal works such as~\cite{LFK05:Liao,liao2007hcr}, Liao et al. demonstrate the prediction and correlation of activities using location information. Eagle and Pentland propose the use of multimodal \textit{eigenbehaviors}~\cite{Eagle2009b} for behaviour prediction. Eigenbehaviors are vectors that describe key characteristics of observed human behaviour over a specified time interval. The vectors are obtained through the principal component analysis (PCA) of a matrix that describes a deviation in sensed features. Besides being a convenient notation for time-variant behaviour, by means of simple Euclidean distance calculation, eigenbehaviors enable direct comparison of behaviour patterns of different individuals. Eagle and Pentland demonstrate the ability of eigenbehviors to recognize  structures in behaviours by identifying different student groups from the Reality Mining data set. 

Anticipatory sensing enables inference of subtle characteristics of human behaviour. In their work on health status prediction, Madan et al. use mobile phone based co-location and communication sensing to measure characteristic behaviour changes in symptomatic individuals~\cite{Madan2010}. The authors find that health status can be predicted with such modalities as calling behaviour, diversity and entropy of face-to-face interactions and user movement patterns. Interestingly, they demonstrate that both physiological as well as mental states can be predicted by the proposed framework. 

Rich psychological context, including user's expectations, cognitive load and flexibility in decision making can be harnessed in mobile computing applications \cite{Bao2013}. Bao et al. show that various domains, such as image compression and video streaming can benefit from psychological context inference. Finally, political opinion fluctuation is a topic of another pioneering work by Madan et al.~\cite{Madan2011a}, which show the potential use of the information collected by mobile sensing systems for understanding and predicting human behavior at scale. In this work call and SMS records, Bluetooth and WiFi environment and  are used to model opinion change during the 2008 presidential elections in the United States. Face-to-face personal encounters, measured through Bluetooth and WiFi collocation, are the key factor in opinion dissemination. The authors also discover patterns of dynamic homophily related to external political events, such as election debates. Automatically estimated exposure explains individual opinions on election day. 

% Non-linear time series analysis is also used by De Domenico et al who exploit movement correlation and social ties for location anticipation \cite{DeDomenico2012}. Harnessing movement traces from users' friends or people with correlated mobility patterns, the authors demonstrate improved accuracy of prediction on the MDC data set.


\subsection{Closing the Feedback Loop -- Context Prediction for Behaviour Change Interventions}
Predicting user behaviour has been connected with mobile phones ever since they became irreplaceable, ubiquitous means of communication, and a need arose for intelligent user interfaces that adapt to individual usage~\cite{Mitrovic2005}. 
Novel applications that bridge the one-way bond between users and computing devices have appeared recently. The goal of these applications is to harness a unique perspective that a personal device has about its user to catalyse positive behavioural change. Merged with the Internet, that has been proposed as a medium for large scale health improvement therapies \cite{Webb2010}, smartphones become a platform for a new type of health and well-being applications called digital behaviour change interventions (dBCIs).
% However, a modern smartphone is much more than a point of contact with the Internet.
 This idea is expressed in~\cite{Lane2010} where the authors call for~\textit{persuasive mobile sensing}. 
 %Unique affordances of smartphones are used as a basis for positive behaviour change. 
 Unlike traditional means of behaviour change interventions, i.e. regular meetings with a therapist, smartphones can deliver tailored feedback about user's behaviour exactly when the feedback is needed, having a stronger persuading power over the user. This way of involvement is termed an~\textit{ecological momentary intervention (EMI)}~\cite{Heron2010}. In addition, smartphone sensing eliminates the need for explicit user querying, since information about user behaviour can be automatically collected. 

Examples of mobile-based EMI systems include UbiFit~\cite{Consolvo2008} and BeWell~\cite{Lane2011b}. In the former a phone's ambient background displays a garden that grows as user's behaviour gets in accordance with predefined physical activity goals. In BeWell, core aspects of physical, social, and mental wellbeing -- sleep, physical activity, and social interactions -- are monitored, and feedback is provided via a mobile phone ambient display. The display shows an aquatic ecosystem where the number and the activity of animals depend on user's wellbeing.  Predicting and impacting human behaviour can be expanded from individuals to groups of users. At MIT research has been done on anticipation of social encounters' outcomes, and with a high reliability inferences can be made of whether conference attendees would exchange business cards, which couples would exchange phone numbers at a bar, and who would come out ahead in a negotiation~\cite{Pentland2005}. Applications that guide the users in their daily lives can be built upon these social outcome predictions. Along the same lines SociableSense examines the socialization network within an enterprise and provides feedback about individual sociability to the group members. Consequently, behaviours change and workers tend to put more effort into healthy socialization \cite{Rachuri2011}. Similarly, SocioPhone monitors turn taking in face-to-face interactions and enables dBCI applications to be designed on top of it \cite{Lee2013}. One such application that the authors propose is SocioTherapist. Designed for autistic children, SocioTherapist presents a game in which a child is rewarded each time it performs a successful turn taking. Social environment is also used as a motivator in \textit{the Social fMRI}, an application that aims to increase physical activity of its users \cite{Aharony2011}. In Social fMRI a close circle of friends get automatic updates whenever an individual phone registers that its user is exercising, promoting a competitive and stimulating environment.

UbiFit and BeWell exploit innovative user interface techniques to close the loop between mobile sensing and behaviour interventions. The ambient display is always present, and each time a phone is used, its owner gets a picture of his or her physical activity and level of sociability. For many other applications that need to deliver an explicit timely advice, interaction with the user is an open problem: if the user has to be notified via SMS, for example, how often should a message be sent, at what time, in which context? These are typical human-computer interaction questions related to interruptibility. In Section~\ref{sec:improvingHCI} we presented some of the related work in this research area.

Finally, the existing dBCI prototypes have been tried on modest user bases. Health related problems that can be tackled through behaviour change therapies, such as diabetes, obesity or smoking, affect hundreds of millions of people. It is not clear if current mobile systems are capable of sustaining dBCIs on such a large scale. In~\cite{Lathia2013} the authors examine challenges in the large-scale dBCI domain, namely processing of large volumes of mobile sensor data, generalizability of behaviour inference, context-specific dissemination of dBCI and privacy issues. The authors note that for large-scale dBCI to become successful it is crucial to empower behaviour therapists with an easy to use tool for dBCI implementation, and present UBhave, a holistic platform for large-scale dBCI design and delivery.

% Predicting calls \cite{Phithakkitnukoon2011}. 
%- Predicting consumer intentions 
%- Personalized information retrieval


==> tex/04_anticipatory_computing.tex <==

\section{Realising the Vision of Anticipatory Mobile Computing}
\label{sec:anticipatory_computing}


In the previous section, we have examined the state of the art and the open challenges related to the problem of anticipating context from sensed data. The remaining aspect for realising the vision of \textit{anticipatory mobile computing} is to design algorithms and mechanisms supporting intelligent decisions based on these predictions. An anticipatory system is defined by Rosen as: ``A system containing a predictive model of itself and/or its environment, which allows it to change state at an instant in accord with the model's predictions pertaining to a later instant"~\cite{Rosen1985}. Anticipation is deeply integrated with intelligence, and biological systems often base decisions for their actions on predictions~\cite{Rosen1985}. These predictions are based on models that evolve over time. Smartphones, developing into cognitive phones, may soon acquire all aspects of intelligent thinking, and use anticipated events as a basis for their functioning~\cite{Campbell2012}. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/overview_figure.pdf}
    \caption{Key stages in the anticipatory mobile computing: collecting sensor data, processing it in order to infer context, predicting future events and finally, using past, present and future to make intelligent decisions.}
    \label{fig:overview}
\end{figure}


%Sensing:
%- energy, processing, balancing local and remote processing
%
%Modelling:
%- which features to select
%- which classifer to use
%- data diversity: personalized or central models
%- getting data labels, co-training
%
%Predicting context:
%- Feedback loop:
%   - How to talk to the user
%   - Large scale challenges (UBhave)
%
%Anticipatory computing:
%- Learning:
%   - exploration vs exploitation
%   - accuracy vs curiosity 

Autonomous intelligent decisions represent the culmination of anticipatory mobile computing. Sensing, inferring and anticipating context are key building blocks that need to be in place before smartphone intelligence develops. In Figure~\ref{fig:overview} we depict stages of anticipatory mobile computing, together with some of the challenges encountered at each of the steps. In spite of phenomenal advances in smartphone hardware, devices are still limited in terms of battery charge, computing and communication resources. Thus, as explained in Section~\ref{sec:sensing_and_modeling_context}, resource efficient sensing and scalable machine learning remain major obstacles in the sensing and context inference phases. Recently, personalization has emerged as an important issue. Large data sets, from projects such as the Reality Mining \cite{Eagle2006} or Nokia MDC \cite{Laurila2012}, showed significant differences among individual behaviours calling for personalized context anticipation models. 

Overcoming the obstacles in anticipatory sensing opens up a new horizon for smartphone applications. As an example, in Figure~\ref{fig:overview} we also sketch a fictional application, inspired by StressSense~\cite{Lu2012}, which harnesses smartphone sensing for proactive stress management. Here, a phone unobtrusively monitors the voice of a busy user, infers current stress levels from voice features, predicts future stress levels based on the user's calendar and then intelligently reschedules meetings so that the anticipated stress level is within healthy boundaries. Equipped with the ability to reason about future and react upon the predictions, a smartphone evolves beyond a cognitive phone, thus becoming an anticipatory device.

\subsection{Learning Anticipatory Systems}

Mobile phones enable a quick \textit{model -- action -- effect} feedback loop for anticipatory sensing. In this section we discuss practicalities of building a model of a target phenomenon and refining it through interaction with the environment.

Models that intelligent beings use for anticipatory decision making are bound to be imperfect. Expecting a rainy day a person may decide to bring an umbrella, but the decision might prove to be a wrong one if the day is sunny in the end. Anticipatory computing systems will also make wrong decisions. Learning from mistakes is a virtue of biological systems, \textit{reinforcement learning} is its counterpart in the machine world \cite{Sutton1998}. In reinforcement learning a system develops a decision model so as to maximize the reward it gets from the environment. Suppose that we want to improve the decision making of the stress relief smartphone application in Figure~\ref{fig:overview}. The application will occasionally reschedule user's meetings. Just like in the biological learning, the consequence will be evaluated, and if the application made a mistake, i.e. if the changes to the schedule turn out to be counterproductive, interfere with user's lifestyle or actually cause more stress for the user, a lesson will be learnt. However, two major issues arise with reinforcement learning in this situation. First, how does the application obtain signals that guide the learning? This can be done by an explicit query to the user, essentially asking the person if he/she is happy with decisions made by the application. Yet, the user may consider frequent querying to be irritating. Another option is to look for implicit signals. For example, monitoring if the user makes changes to the schedule immediately after the application interventions. The second issue comes from the intrinsic need of the reinforcement learning to make mistakes in order to learn from them. If the mistakes are costly, and increasing someone's stress level can surely be costly, the application should be careful about experimenting with decisions made with low confidence.  Thus, there is a tradeoff, commonly known as \textit{the exploitation versus exploration tradeoff}, between improving reinforcement learning models and minimizing negative impact on the user \cite{Sutton1998}. 

Interestingly, learning about the environment does not need to involve explicit probing. A form of learning called \textit{latent learning} happens when a subject is immersed into an unknown environment or a situation without any rewards or punishments associated to them~\cite{Tavris1997}. Despite the lack of obvious incentives for learning, experiments with both humans and animals show that subjects form a cognitive map of the environment solely because they experience the world around them. Later, that cognitive map figures in decision making, essentially behaving as a learnt concept. The artificial implementation of latent learning has been demonstrated by Stolzmann and Butz. In~\cite{Stolzmann2000} the authors designed a robot that, just like in experiments with living rats, relies on latent learning to finds its way around a maze. Latent learning relies on the subject's ability to sense the environment. Immersed in the constant sensing of a large number of modalities mobile phones can bring artificial latent learning to the next level. In the stress relief application example, instead of learning how to reschedule meetings only when a user gives feedback on the proposed schedule, a phone could passively monitor a user's meeting pattern, construct a latent model of events and take it into account even during the first rescheduling instance when the feedback is not yet available. Other approaches that are relevant for learning anticipatory systems are those belonging to the area of so-called probabilistic robotics~\cite{Thrun2005}.

The definition of anticipatory systems calls for environment modelling, not just interaction modelling. While predicting the reward from the environment (i.e., its \textit{action value}) represents the key feature of reinforcement learning, a true anticipatory system should be able to predict the consequence of its interaction on the environment (i.e., the \textit{action effect})~\cite{Lanzi2008}. Initial steps in this area have been made through a machine learning technique termed \textit{anticipatory classifier systems} \cite{Stolzmann1998}.  In such a system the expectation of a future environment state is embedded within classifiers that model the problem. These classifiers are organized in a population that evolves over the course of its interaction with the environment. The evolving collection of classifiers itself is known as the \textit{learning classifier system}, and has been a subject of extensive research, an overview of which can be found in the survey article by Lanzi~\cite{Lanzi2008}. 


%An alternative view on anticipatory computing has been proposed by Holland. In this work, a group of classifiers that evolve over the course of their interaction with the environment has been proposed. Termed \textit{learning classifier systems}, these classifiers represent an evolving population that through genetic operations advances towards more accurate predictions.  This idea has been further extended with \textit{anticipatory classifier systems}, that predict how the problem will evolve after an action has been executed \cite{}. So far anticipatory classifier systems have been successfully applied to robot eye-hand coordination learning, for example. 


%What all of these systems miss is the collective intelligence. 

%\subsection{Scope of Prediction}

Anticipatory systems should be aware of the scope in which they operate and limit their liability to a specific time horizon and events within that scope. The time horizon of anticipation determines how far into future the anticipation goes. Setting the appropriate horizon is of great practical importance. A decision on whether to bring an umbrella or not is useless if made once we are already on the way to work. A decision to bring an umbrella on a day which is a year from now is likely to be inaccurate. Obviously, there is an inherent tradeoff between~\textit{accuracy} and \textit{curiosity} that anticipatory systems have to deal with. Highly proactive behaviour is useful only if the underlying predictions are correct. A sweet spot that determines how far in the future a decision should be made depends on the accuracy of the model, but also on the application for which predictions are made. 
\mm{I had a look at the paper by Dubois, I am not really convinced about these definitions - I suggest to remove them, let's discuss this point. I also think that should be external and not externalist like the author says.}
%Another important aspect of the forecasting scope is the nature of prediction with respect to the events that are anticipated. Thus, anticipation can be externalist or internalist. In the externalist anticipation events that are beyond our control, such as weather conditions, are anticipated. On the other hand, the internalist anticipation predicts events we create ourselves~\cite{Dubois1998}. Despite a considerable interest from the philosophical side, the scope of prediction is yet to be well researched from the practical machine learning side.



%The problem of determining and handling internalist or externalist nature of anticipation remains to be explored. Intuitively, game theory and machine learning techniques could provide initial practical solutions.


%The problem of determining and handling the scope of anticipatory domain and its internalist or externalist nature, remains to be explored. Intuitively, game theory and machine learning techniques could provide initial practical solutions.

%Long-term vs. short-term: The used method should ideally be suitable (e.g. parameterizable) for different forecasting horizons, i.e. predicting context in the near future with high confidence, but also being able to predict later context, most probably with lower confidence.



\subsection{Applications of Anticipatory Mobile Computing}

While theoretical results of anticipatory computing have seen significant advancement in the last three decades, practical applications are lacking. Anticipatory computing has been successfully applied in robotics for eye-hand coordination learning and action planning \cite{Stolzmann2000}, yet the inability to seamlessly interact with the environment and sense feedback that will guide anticipatory learning is the major obstacle for further proliferation of anticipatory computing applications. With smartphones this restriction is lifted. Multimodal sensing and high processing capabilities of modern phones enable full scale anticipatory computing. At the same time, phones' anytime-anywhere use can serve as a basis for novel, highly personalised applications. Anticipatory computing can be applied to a number of mobile sensing sub-domains; here we briefly mention three possible applications:

\begin{itemize}

\item{\textit{Personal assistant technology.} A mobile phone has access to a wealth of personal information, including Web browsing history, calendar events, and online social network contacts. Application developers can tap into it and design applications that can predict the user's intentions and display momentary relevant content. MindMeld is one such application that enhances online video conferencing with information that the users are likely to find relevant in near future~\cite{MindMeld}. For that, MindMeld harnesses real-time speech analysis, machine learning and WWW harvesting. Google Now takes a more general approach and aims to provide a mobile phone user with any information or a functionality she may need, without the user explicitly asking for it~\cite{GoogleNow}. MindMeld and Google Now already live up to the Rosen's definition of the anticipatory system. If augmented with a model that predicts environment's reaction to user's actions these application could become intelligent personal assistants that perform autonomously for user's benefit. Such an application could, for example, foresee an encounter with one's boss, predict the outcome of certain arguments in salary negotiation, and direct the user towards a successful pay raise.}

\item{\textit{Medical services.} Mobile sensing has been proposed as a means for providing in situ diagnosis. In addition, mobile phones are increasingly being used to deliver personalized therapies~\cite{Klasnja2009,Morris2010,Yardley2013}. Currently these therapies tend to be pre-loaded on users phones and react according to the sensed data. Anticipatory computing can be used to build and evolve a model of human behaviour and devise therapies automatically, aiming to get user to a certain well-being goal. Through latent learning, for example, the system can infer how the health issue progresses and adjust the therapy on-the-fly. Such a self-contained application that anticipates changes in user's health and behaviour allows scalability and personalization unimaginable in the traditional physician -- patient world.}

\item{\textit{Smart cities.} The ratio of urban population experiences a steady growth and nowadays more than a half of approximately seven billion people living on Earth reside in urban areas~\cite{WHO2010}. Issues such as traffic, pollution and crime plague modern cities. Participatory mobile sensing, where citizens are actively involved in data collection, as well as opportunistic mobile sensing, where users simply volunteer to host an autonomous application on their devices, have already been employed for tackling urban problems\footnote{For an overview of urban sensing and human-centric sensing research, we refer the reader to~\cite{Campbell2008}, \cite{Srivastava2012} and \cite{EvansCowley2010}.}. MIT's CarTel project uses mobile sensing for traffic mitigation, road surface monitoring and hazard detection \cite{Hull2006}; ParkNet system collects parking space occupancy information through distributed sensing from passing-by vehicles \cite{Mathur2010}; Dutta et al. demonstrated a participatory sensing architecture for monitoring air quality \cite{Dutta2009}. An anticipatory system that makes autonomous decisions and reasons about their consequences can push such projects further. Thus, we envisage a smart navigation system that directs traffic so to alleviate road congestion and balance pollution levels across the city. In addition, people-centric anticipatory mobile computing promises a radical advancement of the way we tackle social problems. Distributed \textit{surveillance}~\cite{Mann2002}, for example based on opportunistic sensing, can be harnessed for early detection of violent riots or terrorist acts. Moreover, through a feedback loop, citizens can be provided with a personalised advice of how to avoid harmful consequences, or organize into first-aid smart mobs~\cite{Rheingold2002}.

%The social side of information networking, Katz
%CreekWatch IBM
%BikeNet
}

\end{itemize}


\subsection{Towards Large-Scale Anticipatory Mobile Computing}
\mm{changed the title for consistency - since we did not explicit talk about "challenges" before}
\mm{Really like this addition!}
%\vp{Adding this to present future challenges. All the other challenges we elaborated quite a lot in the previous sections: energy, processing, balancing local and remote processing, feature and classifier selection, how to interact with the user, learning challenges exploration vs exploitation, etc.}
Applications that rely on anticipatory computing are posed to be inherently more human-like in their behaviour than legacy ones without predictive reasoning. Whether as personal assistants, doctors or even parents, anticipatory applications can provide domain-expert knowledge and personalized advising. Yet, these applications can go even further since, unlike humans, they are not constrained to a single subjective view of a situation. Rather, multiple phones can collaborate  towards common predictions and interactions. Such a large-scale anticipatory mobile computing introduces novel challenges, which can be be summarized as follows:

\begin{itemize}
\item {\textit{Collective sensing and prediction.} High density of sensing devices, including smartphones, wearables and environment sensing networks calls for joint consideration of all the sensing sources when it comes to anticipatory mobile computing. Frameworks for collaborative sensing include AnonySense~\cite{Cornelius2008}, Pogo~\cite{Brouwers2012} and PRISM~\cite{Das2010}. These projects allow application developers to distribute sensing over a large number of mobile devices and process individual devices' sensor data in a centralised way. In Section \ref{sec:large_scale} we already noted that context sensing can harness multiple views of the same event for improved inference. When it comes to context anticipation and intelligent decision making, however, collaboration raises new research questions. Here multiple users do not only observe, but participate in context shaping. Thus, one person's future often depends on anticipated behaviour of another person. This interaction of subjective futures is evident on a simple example of traffic regulation. An intelligent phone might suggest an alternative route when a traffic congestion is anticipated on the usual route. Yet, if everyone involved in the congestion is advised to take the same alternative route, the conditions on which the route calculation is based will change, and the routing suggestions lose their value. }

\item {\textit{Big-data sensing.} We are living in the world of humongous data. We post photos on Facebook, we tweet about our thoughts, we carry smartphones that sense every second of our lives. Traditional methods of understanding human behaviour are insufficient to cope with the growing influx of personalised digital data \cite{Lazer2009}. Sensor data comes in numerous streams that are expensive to store and process offline. Stream processing solutions have been proposed for centrally-managed static sensor networks~\cite{Madden2002}; handling stream processing in the case where data comes from heterogeneous, opportunistic data sources is an open research question. Finally, a large number of sources makes it hard to monitor the quality of a single source. Sensor malfunctioning, malicious participants or the fact that human behaviour might change when the subjects are aware of the sensors~\cite{Davis2012}, can lead to erroneous context inference and prediction.}

\item {\textit{Privacy and anonymity}
Smartphones can provide information about their owner's location, activities, emotions. In addition, phones are, for most of the time, physically close to their users and connected to the global network. Thus, privacy and anonymity breaches in mobile sensing can result in unprecedented leaks of personal data. Lane et al. identify mobile sensing-specific dangers with respect to privacy preservation \cite{Lane2010}. Centralised processing of raw microphone data, for example, while improving voice recognition performance, requires remote handling of sensitive data, which may not be acceptable for some users. Another privacy problem indigenous for mobile sensing stems from mismatched privacy policies over multiple users. For example, if all users volunteer information about other users they are with, but only a subset of users decides to share their GPS coordinates, those users who do not wish to share their GPS data can still have their privacy breached, if they are collocated with those who are willing to report their GPS coordinates. Anticipatory mobile computing exacerbates privacy concerns. Latent learning in an anticipatory computing application can include modelling the behaviour of a person who does use the application herself.\mm{should we give away this idea or not? :) } Differential privacy \cite{Dwork2006}, a concept where one's participation does not increase the risk of privacy breach, has been proposed for privacy-preserving mobility modelling \cite{Isaacman2012}. In anticipatory mobile computing, differential privacy is unlikely to be sufficient, as shown in the previous example.}

\end{itemize} 

%Sensing:
%- 
%
%Modelling:
%- which features to select
%- which classifer to use
%- data diversity: personalized or central models
%- getting data labels, co-training
%
%Predicting context:
%- Feedback loop:
%   - How to talk to the user
%   - Large scale challenges (UBhave)
%
%Anticipatory computing:
%- Learning:
%   - exploration vs exploitation
%   - accuracy vs curiosity 

==> tex/05_conclusion.tex <==
\section{Conclusion}

%Merely five years have passed since Apple released its iPhone. What followed was an unthinkable flurry of innovation in the area of mobile computing. Smartphones are rapidly reaching out into every segment of the society. Mobile broadband has become the single most dynamic ICT service reaching a 40\% annual subscription growth in 2011, and that growth is especially pronounced in the developing world \cite{ITU2012}. Once smartphones penetrate into diverse markets we can expect another wave of culture-specific innovation in the area of mobile sensing.

%In just a decade mobile phones have evolved from merely communication equipment into smart devices capable of extending our senses. In each subsequent generation smartphones are equipped with more and more sensors. With these novel sensing modalities the perception of the world from the point of view of a smartphone reaches beyond the dimensionality defined by our biological senses. Rich computing capabilities and geographically limitless inter-connectivity allow both broad, society-wide, as well as individual context inference. Once we merge advance intelligence capable of making judicious predictions with the above affordances of smartphones, we will set foundations for ubiquitous anticipatory computing and unimaginable applications it may bring.

In this survey we have summarized recent and ongoing efforts in the area of \textit{anticipatory mobile computing}, outlining the open challenges for researchers and practitioners. This field is in continuous evolution. Indeed, merely five years have passed since Apple released its iPhone. In each subsequent generation smartphones have been equipped with more and more sensors. With these novel sensing modalities the perception of the world from the point of view of a mobile device reaches beyond the dimensionality defined by our biological senses. Projects such as Google Glass lead to a true integration between our physical bodies and electronic communication devices we use \cite{GoogleGlass}. In addition, rich computing capabilities and geographically limitless inter-connectivity allow both broad, society-wide, as well as individual context inference. Once we merge advance intelligence capable of making predictions with the above affordances of mobile devices, we will set foundations for ubiquitous anticipatory computing and unimaginable applications it may bring. It is our hope that the path laid out in this article represents a valuable guideline for further efforts in the area of anticipatory mobile sensing.

%\mm{we should add here a discussion of open challenges in my opinion - this might be a separate section too before conclusions}

%Finally, smartphones are rapidly reaching out into every segment of the society. Mobile broadband has become the single most dynamic ICT service topping a 40\% annual subscription growth in 2011, and that growth is especially pronounced in the developing world \cite{ITU2012}. Once smartphones penetrate into diverse markets and reach populations with different needs and behaviours we can expect another wave of culture-specific innovation in the area of mobile sensing.



==> tex/abstract.tex <==
\begin{abstract}
%Today's mobile phones are far from mere communication devices they were ten years ago. Equipped with sophisticated sensors and high power computing hardware, mobile phones can be used to infer user's location, activity, social setting and more. As mobile devices become increasingly intelligent, their capabilities evolve beyond inferring context to anticipating it. In this article we provide an overview of the current state-of-the-art work in predictive mobile sensing. We present a survey of phenomena that mobile phones can infer and predict, and complement it with a description of machine learning techniques used for such predictions. Finally, we discuss the future of anticipatory pervasive computing, outlining the open challenges and a research agenda for the next years. %, specifically how can anticipated events can be used as a basis for smart decision making.
\end{abstract}



==> tex/challenges.tex <==
% challenges
% - learning anticipatory systems
% - towards large scale


\section{Challenges: Realising the Vision}
\label{sec:challenges}

Mobile phones enable a quick \textit{model -- action -- effect} feedback loop for anticipatory sensing. Modelling the environment and the impact that autonomous actions can have on it is a major issue in anticipatory sensing. 



In this section, first, we discuss practicalities of building a model of a target phenomenon and refining it through interaction with the environment. The applications of anticipatory sensing can embrace a holistic view of a situation, in case multiple devices coordinate their actions. In the second part of this section we set the path towards large-scale anticipatory sensing.


%An alternative view on anticipatory computing has been proposed by Holland. In this work, a group of classifiers that evolve over the course of their interaction with the environment has been proposed. Termed \textit{learning classifier systems}, these classifiers represent an evolving population that through genetic operations advances towards more accurate predictions.  This idea has been further extended with \textit{anticipatory classifier systems}, that predict how the problem will evolve after an action has been executed \cite{}. So far anticipatory classifier systems have been successfully applied to robot eye-hand coordination learning, for example. 


%What all of these systems miss is the collective intelligence. 

\subsection{Scope of Anticipation}



Anticipatory systems should be aware of the scope in which they operate and limit their liability to a specific time horizon and events within that scope. The time horizon of anticipation determines how far into future the anticipation goes. Setting the appropriate horizon is of great practical importance. A decision on whether to bring an umbrella or not is useless if made once we are already on the way to work. A decision to bring an umbrella on a day which is a year from now is likely to be inaccurate. Obviously, there is an inherent tradeoff between~\textit{accuracy} and \textit{curiosity} that anticipatory systems have to deal with. Highly proactive behaviour is useful only if the underlying predictions are correct. A sweet spot that determines how far in the future a decision should be made depends on the accuracy of the model, but also on the application for which predictions are made. 

%Long-term vs. short-term: The used method should ideally be suitable (e.g. parameterizable) for different forecasting horizons, i.e. predicting context in the near future with high confidence, but also being able to predict later context, most probably with lower confidence.


\subsection{Towards Large-Scale Anticipatory Mobile Computing}
\mm{changed the title for consistency - since we did not explicit talk about "challenges" before}
\mm{Really like this addition!}
%\vp{Adding this to present future challenges. All the other challenges we elaborated quite a lot in the previous sections: energy, processing, balancing local and remote processing, feature and classifier selection, how to interact with the user, learning challenges exploration vs exploitation, etc.}
Applications that rely on anticipatory computing are posed to be more human-like in their behaviour than legacy ones without predictive reasoning. Whether as personal assistants, doctors or even parents, anticipatory applications can provide domain-expert knowledge and personalized advising. Yet, these applications can go even further since, unlike humans, they are not constrained to a single subjective view of a situation. Rather, multiple phones can collaborate  towards common predictions and interactions. Such a large-scale anticipatory mobile computing introduces novel challenges, which can be be summarized as follows:

\begin{itemize}
\item {\textit{Collective sensing and prediction.} High density of sensing devices, including smartphones, wearables and environment sensing networks calls for joint consideration of all the sensing sources when it comes to anticipatory mobile computing. Frameworks for collaborative sensing include AnonySense~\cite{Cornelius2008}, Pogo~\cite{Brouwers2012} and PRISM~\cite{Das2010}. These projects allow application developers to distribute sensing over a large number of mobile devices and process individual devices' sensor data in a centralised way. In Section \ref{sec:large_scale} we already noted that context sensing can harness multiple views of the same event for improved inference. When it comes to context anticipation and intelligent decision making, however, collaboration raises new research questions. Here multiple users do not only observe, but participate in context shaping. Thus, one person's future often depends on anticipated behaviour of another person. This interaction of subjective futures is evident on a simple example of traffic regulation. An intelligent phone might suggest an alternative route when a traffic congestion is anticipated on the usual route. Yet, if everyone involved in the congestion is advised to take the same alternative route, the conditions on which the route calculation is based will change, and the routing suggestions lose their value. }

\item {\textit{Big-data sensing.} We are living in a world characterised by enormous amounts of data. We post photos on Facebook, we tweet about our thoughts, we carry smartphones that sense every second of our lives. Traditional methods of understanding human behaviour are insufficient to cope with the growing influx of personalised digital data \cite{Lazer2009}. Sensor data comes in numerous streams that are expensive to store and process offline. Stream processing solutions have been proposed for centrally-managed static sensor networks~\cite{Madden2002}; handling stream processing in the case where data comes from heterogeneous, opportunistic data sources is an open research question. Finally, a large number of sources makes it hard to monitor the quality of a single source. Sensor malfunctioning, malicious participants or the fact that human behaviour might change when the subjects are aware of the sensors~\cite{Davis2012}, can lead to erroneous context inference and prediction.}

\item {\textit{Privacy and anonymity}
Smartphones can provide information about their owner's location, activities, emotions. In addition, phones are, for most of the time, physically close to their users and connected to the global network. Thus, privacy and anonymity breaches in mobile sensing can result in unprecedented leaks of personal data. Lane et al. identify mobile sensing-specific dangers with respect to privacy preservation \cite{Lane2010}. Centralised processing of raw microphone data, for example, while improving voice recognition performance, requires remote handling of sensitive data, which may not be acceptable for some users. Another privacy problem indigenous for mobile sensing stems from mismatched privacy policies over multiple users. For example, if all users volunteer information about other users they are with, but only a subset of users decides to share their GPS coordinates, those users who do not wish to share their GPS data can still have their privacy breached, if they are collocated with those who are willing to report their GPS coordinates. Anticipatory mobile computing exacerbates privacy concerns. Latent learning in an anticipatory computing application can include modelling the behaviour of a person who does use the application herself.\mm{should we give away this idea or not? :) } Differential privacy \cite{Dwork2006}, a concept where one's participation does not increase the risk of that party's privacy breach, has been proposed for privacy-preserving mobility modelling \cite{Isaacman2012}. In anticipatory mobile computing, differential privacy is unlikely to be sufficient, since, as shown in the previous example, privacy of non-participating individual can be breached through latent sensing.}

\end{itemize} 


==> tex/context_inference.tex <==
\section{Context Inference: Mobile Sensing and Context Modelling}
\label{sec:context_inference}

% context inference: smartphone sensing and modelling
% - intro (oSec 2 intro) 
% - sensing, modelling, recognising internal states, challenges

Smartphones have evolved from communication devices to perceptive devices capable of inferring context around them. Mobile phone's ability to infer that its user is jogging~\cite{Miluzzo2008}, commuting to work, sleeping \cite{Lane2011b} or even feeling angry \cite{Rachuri2010}, is enabled by two factors.\mm{maybe add references for each of these activities?} First, modern day smartphones are provisioned with sophisticated \textit{senses} and boast high computational power hardware. A today's phone hosts a touch-screen, GPS, accelerometer, gyroscope, proximity and light sensors, high quality microphones and cameras, in addition to a range of communication interfaces, such as WiFi, Bluetooth, 4G/LTE, and a near-field communication (NFC) interface. Multi-core processors and gigabytes of memory allow smartphones to locally handle a large amount of data coming from these senses and extract meaningful context descriptors. The second key factor that enables phones to infer user behaviour is the increasingly ubiquitous and personal usage of mobile phones. Nowadays, the majority of the world's population owns a mobile phone, and these phones are closely integrated with people's lifestyle. Not only are mobile phones, for a large part of a day, physically present with their owners, phones are also used for highly personal purposes such as organizing meetings, navigation, online social networking and e-commerce.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figs/mobile_sensing_overview_figure.pdf}
    \caption{Mobile sensing: from real-world signals to advanced concepts.}
 	\label{fig:mobile_sensing_challenges}
\end{figure}

Monitoring physical environment and building models that connect raw sensed data to high level concepts represent the core of mobile sensing. In this section we investigate issues related to two key aspects of mobile anticipatory sensing system design: context sensing and modelling. Figure~\ref{fig:mobile_sensing_challenges} depicts a classification of these issues. 
%They broadly fall in two categories: context sensing and context modelling. 
The primary goal of context sensing is to provide an interface between the physical world and a mobile device. Modelling context, on the other hand, concentrates on the collected data manipulation and construction of models that infer interesting events or behaviours from the raw samples. In the area of mobile sensing the two categories are intertwined and incomplete without each other. Yet, historically they have evolved independently. In addition, unique challenges are associated with each of the categories, thus in this section we analyse context sensing and context modelling independently.

\subsection{Sensing Context}
%Wearable computing. 
%Learning patterns of activity using real-time tracking

Computing devices can be truly integrated with the everyday life of individuals only if they are cognisant of their environment. Situations and entities that comprise the environment are collectively termed \textit{context}. Context may have numerous aspects: geographical, physical, social, temporal, organizational, to name a few. Context sensing aims at bridging physical stimuli sensed by device's sensors, also known as modalities, and high level concepts that describe a context. Context sensing is a broad area explored by diverse disciplines, predominantly pervasive computing and robotics. Here we present a brief overview of context sensing for mobile devices. 


\subsubsection{Early Mobile Sensing Systems}

Research in mobile sensing commenced long before smartphones hit the market. Initially, inferring the surrounding context had to rely on purpose-built hardware platforms consisting of independent sensors and a processing device, usually a microcontroller or a laptop. These platforms extended the idea of wearable computing with senses that served to bridge the gap between the physical and digital. 

The Sociometer was one of the first examples of a multi-modal mobile sensing platform \cite{Choudhury2003}. The aim of this project was to automatically and unobtrusively learn social network structures. In order to achieve this design goal, the Sociometer obtained information about human contacts through an infra-red (IR) transceiver and a microphone, all connected to the same micro-controller board. For a social contact to be inferred, first, the IR transceiver had to register the presence of another transceiver ID. However, not all encounters could be classified as social in their nature. Thus, microphone data was processed and if a lively conversation was detected, the Sociometer classified the event as a social contact. The Sociometer project demonstrated how the environment of a mobile device can be inferred with a high accuracy. In addition, it ushered into a new kind of interdisciplinary research where traditional social science concepts are experimentally investigated with the help of mobile sensing.

Extending the idea of the Sociometer, researchers at Intel Research and the University of Washington developed the Mobile Sensing Platform (MSP)~\cite{Choudhury2008}. The MSP was designed as a general purpose sensing device, not only for the recognition of social encounters. Compared to the Sociometer, the MSP includes a wider variety of sensors: a microphone, visible light phototransistor, accelerometer, barometer, temperature and humidity sensor, compass and IR transceiver. The justification for such a large number of sensors came from findings that information gathered by multimodal sensors can offset the ambiguities that arise when a single sensor data is used for inference~\cite{Maurer2006}. Moreover, complementary modalities support the recognition of a wide range of contexts. Thus, the MSP allows inference of human activities such as walking, running, taking stairs, cooking, watching TV, and many others. Consequently, the platform was used as a basis for UbiFit, a body sensing application that infers user's physical well being and through a mobile ambient display encourages individuals to be physically active~\cite{Consolvo2008}. With UbiFit and similar applications mobile sensing advanced from inferring user activities to impacting user behaviour, which is the subject of Section~\ref{sec:closing_loop}
 in this survey.

%Other platforms \cite{Bharatula2005}

The Sociometer and the MSP are just two examples of wearable multimodal platforms developed for mobile sensing before smartphones took off. Other notable examples include a low-power context sensing platform developed by Bharatula et al.~\cite{Bharatula2005}, and SenSay~\cite{Siewiorek2003}, a system based on on-body sensors that introduces context-awareness to a user's mobile phone. More examples of wearable sensing platforms can be found in a survey by Pantelopoulos and Bourbakis~\cite{Pantelopoulos2010}. Common characteristics of all the above platforms is that they included wearable sensors and a separate data processing device, e.g. a laptop, PDA or micro-controller, and were used for collecting data in well planned experiments. Built for only one purpose -- to collect sensor data -- these systems were significantly different than today's smartphones. Nevertheless, wearable platforms demonstrated that mobile sensing became an irreplaceable tool for monitoring and understanding human behaviour. 

\subsubsection{Obstacles to Smartphone-Based Mobile Context Sensing}

The need for custom built sensing platform wanes, as today's smartphones avail highly multimodal sensing, and are unobtrusively carried by their owners at all times. However, applications that use smartphone sensing are still subject to standard mobile sensing constraints identified in earlier work on custom sensing platforms ~\cite{Choudhury2003,Choudhury2008}. Resource-constrained challenges have been the focus of the research agenda of many projects, starting from the first mobile sensing prototypes, such as CenceMe~\cite{Miluzzo2008} and BeTelGeuse~\cite{betelgeuse}. These constraints come from the battery, processing, storage and communication restrictions of smartphone devices. 

\textbf{Energy-efficient operation.}  Energy shortage issues are exacerbated by the design of smartphone sensors as occasionally used features, rather than constantly sampled sensors. A sensing device can reduce its energy consumption either by sampling less often or, in case it hosts multiple sensor types, by preferring low-power sensors to more power hungry ones. Both approaches come with drawbacks of either completely missing to sense important events or sensing them with an insufficient resolution. %Here we present two of the most common ways of addressing energy shortage, as well as a few innovative approaches to energy efficiency in mobile sensing.

SociableSense is a mobile application that senses socialization among users \cite{Rachuri2011}. This system operates on commodity phones and achieves energy efficiency by adapting the sampling rate. A linear reward-inaction function is associated with the sensing cycle, and the rate is reduced during ``quite" times, when no interesting events are observed. The approach is very efficient with human interaction inference, since the target events, i.e., conversations, are not sudden and short. On another side of the solution spectrum Energy Efficient Mobile Sensing System (EEMSS) proposed by Wang et al. hierarchically orders sensors with respect to their energy consumption, and activates high-resolution power-hungry sensors, only when low-consumption ones sense an interesting event~\cite{Wang2009}. The management of sensor states and transitions in EEMSS is performed through an XML styled state descriptor that allows the operator to define interesting events and the desired power saving schemes. The Jigsaw sensing engine~\cite{Lu2010} preserves power by triggering power hungry stages of sensing and sensor data processing only when these become necessary for successful tracking of user behaviour. For example, Jigsaw discards data sensed by a microphone if the intensity of the samples is below a certain intensity threshold. Similarly, a Markov decision process controls GPS sampling such that the sensing rate is increased when a user moves rapidly, and decreased if the movement is slow. 

Location and movement inference is especially interesting from the adaptive sensing perspective, as inferring the exact coordinates of a person is seldom of direct interest compared to inferring a meaningful description of the location (i.e. a coffee shop, home, university campus). In addition, the GPS sensor is one of the most power hungry sensors on a mobile device, and reducing its sampling rate represents an attractive way to increase energy-efficiency of an application \cite{Kim2010}. SensLoc goes beyond the exact coordinate tracking and  recognises important places and paths taken by a user. It relies on a change in the WiFi environment signature in order to detects entrance to or departure from a location. SensLoc further preserves energy by sampling GPS only for path tracking, and only when the phone's accelerometer detects that the user is moving. For trajectory tracking Kjaergaard et al. propose adaptive sampling of accelerometer, compass and GPS sensors in order to achieve the most energy efficient trajectory tracking with the given error tolerance \cite{Kjargaard2011}. The same work also presents a method for simplified trajectory representation. The identification of the minimal model of a phenomena that we are sensing optimises both sensing energy, but also associated storage and communication overheads. 

Humans are creatures of habit and a historical information about their movement can be harnessed for current whereabouts inference. Paek et al. use historical data to guide RAPS, their location sampling algorithm, in an energy-efficient way \cite{Paek2010}. GPS signal is often unreliable in urban areas and unavailable indoors. RAPS uses cell tower blacklisting to quickly recognise areas where GPS was observed to be unusable.  In addition, RAPS estimates user velocity, using a duty-cycled accelerometer, and adaptively turns GPS only if the  estimated uncertainty in position exceeds the accuracy threshold. Identifying patterns in human behaviour can serve as a basis for energy-efficient context inference. A location determination system CAPS relies on the fact that a large number of people tend to take the same route, i.e. daily commute, to minimise GPS sampling for re-visited paths \cite{Paek2011}. This hints an opportunity for interesting multimodal sensing efficiency optimisation. For example, can we optimise location sampling by extracting information from the user's digital calendar? 

The inherent structure of the context inference problem can also be used to improve sensing efficiency. This is the main idea behind the Acquisitional Context Engine (ACE) proposed in \cite{Nath2012}. Here, Nath develops a speculation-based sensing engine that learns associative rules among contexts, an example of which would be ``when a user state is \textit{driving}, his location is not \textit{at home}". When a context-sensitive application needs to know if a user is is at home or not, it contacts ACE that acts as a middle layer between sensors and the application. ACE initially probes a less energy costly sensor -- accelerometer -- and only if the sensed data does not imply that a user is driving, it turns the GPS on and infers the actual user's location. While demonstrated on simple rules, Nath argues that ACE can be complemented with tools that examine the temporal continuity of context, such as SeeMon \cite{Kang2008} to extract sophisticated rules like ``if a user is \textit{at home} now, he cannot be \textit{in the office} in the next ten minutes".

Cloud computing opens up additional opportunities for improved use of energy resources. Let us consider GPS for example. The location is determined through processing of signals received from Global Navigation Satellite System (GNSS) satellites. Because of a low data rate between a satellite and a device, and complex wireless signal processing, required due to Doppler frequency shifts and weak signal strengths, GPS remains on of the most power hungry sensors in mobile phones. In \cite{Liu2012}, the authors develop CO-GPS -- a system where once it gets detected by a mobile device, raw received signals are uploaded to the cloud for processing, relieving a battery limited device from the burden of computation. CO-GPS consumes up to three orders of magnitude less energy than the conventional GPS system. The drawback is that due to increased communication latitude and longitude determination via CO-GPS lags behind the standard GPS approach. Nevertheless, energy efficient operation through offloading from a mobile phone to a cloud is potentially applicable to other sensing modalities where computation energy is greater than energy needed for cloud uploading. Such modalities most likely include those where complex signal processing is needed, e.g. sound and video. At the same time, these modalities come with overwhelming amounts of raw data, transport of which requires high connection quality, and can incur monetary charges to a user. Han and Philipose argue that only intermediate computation steps, such as feature extractors and models will be transferred in an ecosystem of mobile devices, while the advances in hardware will make on-device processing powerful enough to eliminate the need for fully cloud-based solutions \cite{Han2013}.

% Compression sensing?
\textbf{Processing, storage and communication efficiency.} Despite ongoing technological advances mobile phones still have limited processing and data storage capabilities. As mentioned above, remote resources available via online cloud computing can be used to help with data processing. However, the transfer of the high-volume data produced by mobile sensors can be costly, especially if done via a cellular network. 

Balancing local and remote processing was tackled in one of the first smartphone sensing applications, CenceMe~\cite{Miluzzo2008}. This application performs audio and activity classification on the phone, while some other modalities, such as user's location, are classified on a remote server. The distribution of the computation is not performed solely because of the limited computation resources of a smartphone. Distributed computation also allows for aggregation of data from multiple phones, therefore a larger context can be inferred. \ignore{In CenceMe an ``Am I Hot" classifier of user's social behaviour is developed thanks to distributed, multi-user sensing. }Different costs associated with local and remote data processing are examined in SociableSense~\cite{Rachuri2011}. The split between the two is done on the basis of energy expenditure, data transmission cost, and the computation delay. The decision is made when each of the aspects, available energy, data transfer cost and computation latency, are evaluated through a multi-criteria utility function. Each of the aspects figures in the utility function with a certain weight. An XML-based interface is provided through which one can set simple rules that guide weight adjustment. For example, the energy saving can be given the priority if the battery level is low. Custom-made application execution partitioning, such as the one used in CenceMe and SociableSense, requires significant effort from the developer's side. More general solutions allow an application developer to delegate the partitioning task to a dedicated middleware. MAUI, for example, supports fine-grained code offloading to a cloud in order to maximize energy savings on a mobile device \cite{Cuervo2010}. MAUI harnesses code portability, programming reflection and serialisation to automate code partitioning and at runtime decide which methods should be executed in a cloud. The main motivation for the partitioning is again computation energy efficiency. %Conceptually similar, but implementation-wise different solution is CloneCloud~\cite{Chun2011}.

Certain hardware limitations that hamper mobile sensing, most notably the lack of computing capabilities, are likely to be overcome in near future, Modern cellphones already host multi-core processors and gigabytes of memory. Battery related issues, on the other hand, still represent a significant burden to continuous sensing. Distributed mobile sensing brings new, socially-aware, applications, but with additional challenges of data management. We discuss large-scale mobile sensing challenges in Section~\ref{sec:large_scale}

%
%
%%IN PREVIOUS SURVEY PAPERS:
%%+ sensing towards cognitive phones
%%- apps: transportation, environment, health, social nets
%%+ app stores
%%+ scaling
%%- programmability 
%%+ continuous sensing
%%+ crowd-sourcing
%%- human behaviour and context modelling 
%%- sharing via OSNs
%%+ personalized sensing
%%- persuasive computing
%%- predict social outcomes, group dynamic, personal relationships.
%
%Smartphones have evolved from communication devices to perceptive devices capable of inferring context around them. Mobile phone's ability to infer that its user is jogging~\cite{Miluzzo2008}, commuting to work, sleeping \cite{Lane2011b} or even feeling angry \cite{Rachuri2010}, is enabled by two factors.\mm{maybe add references for each of these activities?} First, modern day smartphones are provisioned with sophisticated \textit{senses} and boast high computational power hardware. A today's phone hosts a touch-screen, GPS, accelerometer, gyroscope, proximity and light sensors, high quality microphones and cameras, in addition to a range of communication interfaces, such as WiFi, Bluetooth, 4G/LTE, and a near-field communication (NFC) interface. Multi-core processors and gigabytes of memory allow smartphones to locally handle a large amount of data coming from these senses and extract meaningful context descriptors. The second key factor that enables phones to infer user behaviour is the increasingly ubiquitous and personal usage of mobile phones. Nowadays, the majority of the world's population owns a mobile phone, and these phones are closely integrated with people's lifestyle. Not only are mobile phones, for a large part of a day, physically present with their owners, phones are also used for highly personal purposes such as organizing meetings, navigation, online social networking and e-commerce.
%
%If two or more devices
%have similar sensors, their samples can be merged to
%obtain a possibly more complete view on the
%environment. This has been proposed independently
%in [23],J. Mäntyjärvi, J. Himberg, and P. Huuskonen.
%Collaborative context recognition for handheld
%devices. In First IEEE International Conference on
%Pervasive Computing and Communications
%(PerCom’03), pages 161-168,

\subsection{Modeling Context}
\label{sec:modeling_context}

Raw sensor data, such as those from phone's accelerometer, are seldom of direct interest and machine learning techniques are usually employed to infer higher level concepts, for example, a user's physical activity \cite{Tapia2007}. For the inference to be made, first we need to decide which aspects of the raw sensor data are the most representative of the phenomena we would like to explain. Then, appropriate machine learning techniques are used to build a faithful model of human behaviour and train it with the data gathered so far. Finally, the current context is inferred from the collected data.

\subsubsection{Selecting Useful Modalities and Features from Sensor Data}
\label{sec:select_features}
The first challenge in context modelling is the identification of those modalities of raw data that are the most descriptive of the context. Interdisciplinary efforts and domain knowledge are crucial in this step. For example, if we try to infer user's emotions, the existing work in psychology tells us that emotions are manifested in a person's speech \cite{Bezooijen1983}. Consequently, we can discard irrelevant modalities and concentrate our efforts on processing microphone data.

The next step includes the selection of the appropriate representation for the sensor data. Consider EmotionSense, an experimental psychology research application, which harnesses the fact that a mobile phone microphone can record sufficient information needed for emotion inference \cite{Rachuri2010}. Before the classification, however, raw microphone data has to be transformed to a suitable form. Distinctive properties extracted from the data are called \textit{features}. The EmotionSense authors built its speech recognition models on Perceptual Linear Predictive (PLP) coefficients, a well established approach to speech analysis \cite{Hermansky1990}. An alternative, but less sophisticated means of microphone data manipulation that has proven successful in mobile sensing is the Discrete Fourier Transform (DFT) \cite{Miluzzo2008}. The majority of speech energy is found in a relatively narrow band from 250 Hz to 600 Hz, thus the investigation of DFT coefficient means and variations can help identify speech in an audio trace. Finally, Mel-Frequency Cepstral Coefficients (MFCC) are another commonly used feature for speech recognition \cite{Lu2009,Miluzzo2010,Chon2012}.

\begin{table}[htb]
%\figsp
\caption{Context sensing domains and characteristic features.}
\label{tab:features}
\begin{center}
\begin{scriptsize}
\begin{tabular}{|c|l|}
\hline
\textbf{Domain} & \textbf{Characteristic Features} \\
\hline
\hline
Speech recognition & 
\begin{tabular}[l]{@{}l@{}} -- Sound spectral entropy, RMS, zero crossing rate, low energy frame rate,\\
 spectral flux, spectral rolloff, bandwidth, phase deviation\\
\cite{Lu2009,Lane2011b}\\
-- Mel-Frequency Cepstral Coefficients (MFCCs)\\
\cite{Lu2009,Miluzzo2010,Chon2012,Lu2010,Lu2012}\\
-- Teager Energy Operator (TEO), pitch range, jitter and standard deviation,\\
spectral centroid, speaking rate, high frequency ratio\\
\cite{Lu2012,Lu2010}\\
-- Running average of amplitude, sum of absolute differences\\
\cite{Krause2006}\\
-- Perceptual linear predictive (PCP) coefficients\\
\cite{Rachuri2010}\\
-- Mean and standard deviation of DFT power\\
\cite{Miluzzo2008}


%MFCC, Teager Energy Operator (TEO), Pitch range, jitter and stdev, Spectral centroid, speaking rate, high frequency ratio Lu2012, Lu2010 (without TEO)
%Running average of amplitude, SAD KRause2006
%Sound: Spectral entropy, RMS, zero crossing rate, low energy frame rate,spectral flux, spectral rolloff, bandwidth, phase deviation Lu2009, Lane2011b
%Speech: auto correlation, spectral entropy Choudhury2003
%HMM + MFCC Chon2012
%Music: GMM + MFCC Chon2012
%MFCC - Miluzzo2010
%Mean+ STDEV of DFT power Miluzzo2008
%Perceptual linear predictive (PLP) coefficients  Rachuri2010

\end{tabular}\\
\hline
Activity classification & 
\begin{tabular}[l]{@{}l@{}}-- Accelerometer FFT principal component analysis (PCA)\\
\cite{Krause2006}\\
-- Accelerometer intensity/energy/mean\\
\cite{Eston1998,Lu2010,Rabbi2011,Abdullah2012}\\
-- Accelerometer variance\\
\cite{Miluzzo2008,Lu2010,Rabbi2011,Aharony2011}\\
-- Accelerometer peaks/mean crossing rate\\
\cite{Miluzzo2008,Lu2010}\\
-- Accelerometer spectral features\\
\cite{Lu2009,Lu2010,Lane2011b,Rabbi2011}\\
-- Accelerometer correlations\\
\cite{Abdullah2012}\\
-- Accelerometer frequency domain entropy\\
\cite{Abdullah2012}\\
-- Barometric pressure\\
\cite{Rabbi2011}

\end{tabular}\\
\hline

Location & 
\begin{tabular}[l]{@{}l@{}}
-- Days on which any cell tower was contacted,
days on which a specific tower is contacted, \\
contact duration, events during work/home hours\\
\cite{Isaacman2011}\\
-- Tanimoto Coefficient of WiFi fingerprints \\
\cite{Chon2012}\\
-- Eigenbehaviors - vectors of time-place pairs\\
\cite{Eagle2009b}\\
-- Hour of day, latitude, longitude, altitude, social ties\\
\cite{DeDomenico2012}\\
\end{tabular}\\
\hline
Object recognition & \begin{tabular}[l]{@{}l@{}}-- GIST features\\
\cite{Chon2012}
\end{tabular}\\
\hline
Gestures & \begin{tabular}[l]{@{}l@{}}-- Mean, max, min, median, amplitude, and
high pass filtered values of acc. intensity and jerk;\\
spectral features; screen touch location, slope, speed,
strokes number, length, slope and location\\
\cite{Coutrix2012}\\
\end{tabular}\\
\hline
Physiological state & \begin{tabular}[l]{@{}l@{}}-- Galvanic skin response, heat flux,\\
skin thermometer running average and sum of absolute differences\\
\cite{Krause2006}\\
\end{tabular}\\
\hline
Thoughts & \begin{tabular}[l]{@{}l@{}}-- Bandpass filtered neural signal from EEG\\
\cite{Campbell2010}\\
\end{tabular}\\
\hline
Call prediction & \begin{tabular}[l]{@{}l@{}}--  Call arrival and inter-departure time, calling reciprocity\\  \cite{Phithakkitnukoon2011}\\
\end{tabular}\\
\hline
Interruptibility & \begin{tabular}[l]{@{}l@{}}-- User typing, moving, clicking, application focus, app. activity, gaze, time of day,\\
day of week, calendar, acoustic energy, WiFi environment,\\
\cite{Horvitz2003}\\
-- Mean, energy, entropy and correlation of accelerometer data\\
\cite{Ho2005}
\end{tabular}\\
\hline
\end{tabular}
\end{scriptsize}

\end{center}
\end{table}

%
%Monitoring physical environment and building models that connect raw sensed data to high level concepts represent the core of mobile sensing. In this section we investigate issues related to two key aspects of mobile anticipatory sensing system design: context sensing and modelling. Figure~\ref{fig:mobile_sensing_challenges} depicts a classification of these issues. 
%%They broadly fall in two categories: context sensing and context modelling. 
%The primary goal of context sensing is to provide an interface between the physical world and a mobile device. Modelling context, on the other hand, concentrates on the collected data manipulation and construction of models that infer interesting events or behaviours from the raw samples. In the area of mobile sensing the two categories are intertwined and incomplete without each other. Yet, historically they have evolved independently. In addition, unique challenges are associated with each of the categories, thus in this section we analyse context sensing and context modelling independently.
%
%\subsection{Sensing Context}
%%Wearable computing. 
%%Learning patterns of activity using real-time tracking
%
%Computing devices can be truly integrated with the everyday life of individuals only if they are cognisant of their environment. Situations and entities that comprise the environment are collectively termed \textit{context}. Context may have numerous aspects: geographical, physical, social, temporal, organizational, to name a few. Context sensing aims at bridging physical stimuli sensed by device's sensors, also known as modalities, and high level concepts that describe a context. Context sensing is a broad area explored by diverse disciplines, predominantly pervasive computing and robotics. Here we present a brief overview of context sensing for mobile devices. 
%
%
%\subsubsection{Early Mobile Sensing Systems}
%
%Research in mobile sensing commenced long before smartphones hit the market. Initially, inferring the surrounding context had to rely on purpose-built hardware platforms consisting of independent sensors and a processing device, usually a microcontroller or a laptop. These platforms extended the idea of wearable computing with senses that served to bridge the gap between the physical and digital. 
%
%The Sociometer was one of the first examples of a multi-modal mobile sensing platform \cite{Choudhury2003}. The aim of this project was to automatically and unobtrusively learn social network structures. In order to achieve this design goal, the Sociometer obtained information about human contacts through an infra-red (IR) transceiver and a microphone, all connected to the same micro-controller board. For a social contact to be inferred, first, the IR transceiver had to register the presence of another transceiver ID. However, not all encounters could be classified as social in their nature. Thus, microphone data was processed and if a lively conversation was detected, the Sociometer classified the event as a social contact. The Sociometer project demonstrated how the environment of a mobile device can be inferred with a high accuracy. In addition, it ushered into a new kind of interdisciplinary research where traditional social science concepts are experimentally investigated with the help of mobile sensing.
%
%Extending the idea of the Sociometer, researchers at Intel Research and the University of Washington developed the Mobile Sensing Platform (MSP)~\cite{Choudhury2008}. The MSP was designed as a general purpose sensing device, not only for the recognition of social encounters. Compared to the Sociometer, the MSP includes a wider variety of sensors: a microphone, visible light phototransistor, accelerometer, barometer, temperature and humidity sensor, compass and IR transceiver. The justification for such a large number of sensors came from findings that information gathered by multimodal sensors can offset the ambiguities that arise when a single sensor data is used for inference~\cite{Maurer2006}. Moreover, complementary modalities support the recognition of a wide range of contexts. Thus, the MSP allows inference of human activities such as walking, running, taking stairs, cooking, watching TV, and many others. Consequently, the platform was used as a basis for UbiFit, a body sensing application that infers user's physical well being and through a mobile ambient display encourages individuals to be physically active~\cite{Consolvo2008}. With UbiFit and similar applications mobile sensing advanced from inferring user activities to impacting user behaviour~\cite{Lathia2013}.
%
%%Other platforms \cite{Bharatula2005}
%
%The Sociometer and the MSP are just two examples of wearable multimodal platforms developed for mobile sensing before smartphones took off. Other notable examples include a low-power context sensing platform developed by Bharatula et al.~\cite{Bharatula2005}, and SenSay~\cite{Siewiorek2003}, a system based on on-body sensors that introduces context-awareness to a user's mobile phone. More examples of wearable sensing platforms can be found in a survey by Pantelopoulos and Bourbakis~\cite{Pantelopoulos2010}. Common characteristics of all the above platforms is that they included wearable sensors and a separate data processing device, e.g. a laptop, PDA or micro-controller, and were used for collecting data in well planned experiments. Built for only one purpose -- to collect sensor data -- these systems were significantly different than today's smartphones. Nevertheless, wearable platforms demonstrated that mobile sensing became an irreplaceable tool for monitoring and understanding human behaviour. 
%
%\subsubsection{Obstacles to Mobile Context Sensing}
%
%The need for custom built sensing platform wanes, as today's smartphones avail highly multimodal sensing, and are unobtrusively carried by their owners at all times. However, applications that use smartphone sensing are still subject to standard mobile sensing constraints identified in earlier work on custom sensing platforms ~\cite{Choudhury2003,Choudhury2008}. Resource-constrained challenges have been the focus of the research agenda of many projects, starting from the first mobile sensing prototypes, such as CenceMe~\cite{Miluzzo2008} and BeTelGeuse~\cite{betelgeuse}.
%
%These constraints come from the battery, processing, storage and communication constraints of mobile devices. Energy shortage issues are exacerbated by the design of smartphone sensors as occasionally used features, rather than constantly sampled sensors. A sensing device can reduce its energy consumption either by sampling less often or, in case it hosts multiple sensor types, by preferring low-power sensors to more power hungry ones. Both approaches come with drawbacks of either completely missing to sense important events or sensing them with an insufficient resolution. Here we present two of the most common ways of addressing energy shortage, as well as a few innovative approaches to energy efficiency in mobile sensing.
%
%SociableSense is a mobile application that senses socialization among users \cite{Rachuri2011}. This system operates on commodity phones and achieves energy efficiency by adapting the sampling rate. A linear reward-inaction function is associated with the sensing cycle, and the rate is reduced during ``quite" times, when no interesting events are observed. The approach is very efficient with human interaction inference, since the target events, i.e., conversations, are not sudden and short. On another side of the solution spectrum Energy Efficient Mobile Sensing System (EEMSS) proposed by Wang et al. hierarchically orders sensors with respect to their energy consumption, and activates high-resolution power-hungry sensors, only when low-consumption ones sense an interesting event~\cite{Wang2009}. The management of sensor states and transitions in EEMSS is performed through an XML styled state descriptor that allows the operator to define interesting events and the desired power saving schemes. The Jigsaw sensing engine~\cite{Lu2010} preserves power by triggering power hungry stages of sensing and sensor data processing only when these become necessary for successful tracking of user behaviour. Therefore, Jigsaw discards data sensed by a microphone if the intensity of the samples is below a certain intensity threshold. Similarly, a Markov decision process controls GPS sampling such that the sensing rate is increased when a user moves rapidly, and decreased if the movement is slow. 
%
%The inherent structure of the context inference problem can be used to improve sensing efficiency. This is the main idea behind the Acquisitional Context Engine (ACE) proposed in \cite{Nath2012}. Here, Nath develops a speculation-based sensing engine that learns associative rules among contexts, an example of which would be ``when a user state is \textit{driving}, his location is not \textit{at home}". When a context-sensitive application needs to know if a user is is at home or not, it contacts ACE that acts as a middle layer between sensors and the application. ACE initially probes a less energy costly sensor -- accelerometer -- and only if the sensed data does not imply that a user is driving, it turns the GPS on and infers the actual user's location. While demonstrated on simple rules, Nath argues that ACE can be complemented with tools that examine the temporal continuity of context, such as SeeMon \cite{Kang2008} to extract sophisticated rules like ``if a user is \textit{at home} now, he cannot be \textit{in the office} in the next ten minutes".
%
%Cloud computing opens up additional opportunities for improved use of energy resources. Let us consider GPS for example. The location is determined through processing of signals received from Global Navigation Satellite System (GNSS) satellites. Because of a low data rate between a satellite and a device, and complex wireless signal processing, required due to Doppler frequency shifts and weak signal strengths, GPS remains on of the most power hungry sensors in mobile phones. In \cite{Liu2012}, the authors develop CO-GPS -- a system where once it gets detected by a mobile device, raw received signals are uploaded to the cloud for processing, relieving a battery limited device from the burden of computation. CO-GPS consumes up to three orders of magnitude less energy than the conventional GPS system. The drawback is that due to increased communication latitude and longitude determination via CO-GPS lags behind the standard GPS approach. Nevertheless, energy efficient operation through offloading from a mobile phone to a cloud is potentially applicable to other sensing modalities where computation energy is greater than energy needed for cloud uploading. Such modalities most likely  include those where complex signal processing is needed, e.g. sound and video. %However, restrictions on the answer delay and the cost of communication make 
%
%
%% Compression sensing?
%
%Despite ongoing technological advances mobile phones still have limited processing and data storage capabilities. As mentioned above, remote resources available via online cloud computing can be used to help with data processing. However, the transfer of the high-volume data produced by mobile sensors can be costly, especially if done via a cellular network. 
%
%Balancing local and remote processing was tackled in one of the first smartphone sensing applications, CenceMe~\cite{Miluzzo2008}. This application performs audio and activity classification on the phone, while some other modalities, such as user's location, are classified on a remote server. The distribution of the computation is not performed solely because of the limited computation resources of a smartphone. Distributed computation also allows for aggregation of data from multiple phones, therefore a larger context can be inferred. In CenceMe an ``Am I Hot" classifier of user's social behaviour is developed thanks to distributed, multi-user sensing. Different costs associated with local and remote data processing are examined in~\cite{Rachuri2011}. The split between the two is done on the basis of energy expenditure, data transmission cost, and the computation delay. The decision is made when each of the aspects, available energy, data transfer cost and computation latency, are evaluated through a multi-criteria utility function. Each of the aspects figures in the utility function with a certain weight. An XML-based interface is provided through which one can set simple rules that guide weight adjustment. For example, the energy saving can be given the priority if the battery level is low. 
%
%Certain hardware limitations that hamper mobile sensing, most notably the lack of computing capabilities, are likely to be overcome in near future, Modern cellphones already host multi-core processors and gigabytes of memory. Battery related issues, on the other hand, still represent a significant burden to continuous sensing. Distributed mobile sensing brings new, socially-aware, applications, but with additional challenges of data management. 
%
%%
%%\subsubsection{Sensing on Multiple Devices}
%%
%%Types of mobile sensing: particpatory, opportunitstic.
%%
%%
%%If two or more devices
%%have similar sensors, their samples can be merged to
%%obtain a possibly more complete view on the
%%environment. This has been proposed independently
%%in [23],J. Mäntyjärvi, J. Himberg, and P. Huuskonen.
%%Collaborative context recognition for handheld
%%devices. In First IEEE International Conference on
%%Pervasive Computing and Communications
%%(PerCom’03), pages 161-168,
%
%\subsection{Modeling Context}
%\label{sec:modeling_context}
%
%Raw sensor data, such as those from phone's accelerometer, are seldom of direct interest and machine learning techniques are usually employed to infer higher level concepts, for example, a user's physical activity \cite{Tapia2007}. For the inference to be made, first we need to decide which aspects of the raw sensor data are the most representative of the phenomena we would like to explain. Then, appropriate machine learning techniques are used to build a faithful model of human behaviour and train it with the data gathered so far. Finally, the current context is inferred from the collected data.
%
%\subsubsection{Selecting Useful Modalities and Features from Sensor Data}
%\label{sec:select_features}
%The first challenge in context modelling is the identification of those modalities of raw data that are the most descriptive of the context. Interdisciplinary efforts and domain knowledge are crucial in this step. For example, if we try to infer user's emotions, the existing work in psychology tells us that emotions are manifested in a person's speech \cite{Bezooijen1983}. Consequently, we can discard irrelevant modalities and concentrate our efforts on processing microphone data.
%
%Object recognition: GIST features (FIND REF!) Chon2012

The above discussion shows that numerous features can be extracted from a single modality. In many domains, however, certain feature types have crystallized out as the most informative. Table~\ref{tab:features} lists the most commonly observed features and the domains in which they are used. The table is not meant to be a comprehensive survey of feature extraction, but should point out that even with a small number of sensors there can be hundreds of possible features all of which may or may not contribute to context inference~\cite{Choudhury2008}. To tackle the problem of feature selection one possibility is to employ computationally inexpensive mathematical transformation known as the Principle Component Analysis (PCA)~\cite{Pearson1901}, as demonstrated in~\cite{Krause2006}. After the PCA is performed we are left with a set of most promising features that impact the target variable the most, i.e., in this case the aspect that we want to infer. However, different classifiers might give different results even with the same features. Wrapping is used as a more accurate, albeit more computationally complex, alternative to PCA~\cite{Kohavi1997}. In this procedure, based on the collected data, a classifier is built with each of the subsets of features. A part of the data is left out during the training phase and is used to evaluate the classifiers. An example of wrapping based feature selection can be found in the human interruption study by Fogarty et al.~\cite{Fogarty2005}. A boosting-based technique for ranking features according to their contribution towards context recognition has been proposed by Lester et al.~\cite{Lester2005}. Their approach iteratively trains an ensemble of weak binary classifiers constrained to use a single feature each. At the end of the training we are left with not only the ranking of features, but also with the weights that indicate how important each of the features is for the final classification. Interestingly, the same classifier, used in different environments, may require different features for successful classification. For example, a standard speech classification attribute MFCC does not perform well outdoors while more noise tolerant features, such as high frequency energy ratio and frequency centroid become more discriminative in this setting~\cite{Lu2012}.

Modality and feature selection impact the rest of the context inference; a careful consideration at this stage of the process can help improve classification accuracy or reduce the computational complexity of the learning process. As mobile sensing matures the variety of context types that we strive to infer broadens. In addition, the number of sensors available on the smartphone increases steadily. Therefore, identifying and quantifying the strength of a link between a domain and a modality (or a feature) emerges as an important research direction in mobile sensing.
%With an increasing number of sensors and a growing interest in a variety of context domains, identifying and quantifying the strength of a link between a domain and a modality or a feature emerges as an important research direction in mobile sensing.
%Unfortunately, in many domains we still cannot answer a question of whether a link between a concept and a modality or a feature can be established.\mm{This comment might sound a bit vague - perhaps add more details}


\subsubsection{Classification Methods}
\label{sec:classification_methods}
The construction of models is a crucial part of the design of context inference systems. A plethora of machine learning techniques at our disposal can be used to transfer distilled sensor data into mathematical representations of user behaviour. In this survey we concentrate on a small subset of machine learning techniques that have been successfully applied to mobile sensing problems, and we refer an interested reader to machine learning texts such as, for example,~\cite{Bishop2006,elementsstatisticallearning2009,RG11:first,Bar12:Bayesian}.

We examine how context inference models are built in case of StressSense, mobile phone application that analyses speech data collected via a built-in microphone and identifies if a user is under stress \cite{Lu2012}. The first step in StressSense is sound and speech detection. The application assumes that sound is present if high audio level is present in at least 50 out of 1000 samples taken within a half a second period. In such a case, StressSense divides the audio signal into frames and for each of the frames calculates its zero crossing rate (ZCR) and root mean square (RMS) of the sound. These features correspond to sound pitch and energy. A tree-based classifier that decides between speech and non-speech frames is built with ZCR and RMS as attributes. Further, thresholds on ZCR and spectral entropy are used to discern between voiced and unvoiced frames of human speech. Finally, Gaussian Mixture Models (GMMs) are built for the two target classes -- stressed speech and neutral speech. Pitch, Teager Energy Operator (TEO) and Mel-Frequency Cepstral Coefficient (MFCC) based features of each voiced frame are used for user stress inference.\vp{Added example, consistent with the previous subsection that also has an example.}

The variety of classification methods and data features opens up wide opportunities for novel context inference methods. To help a system designer with the selection of a context inference approach, in Table~\ref{tab:learners} we list mobile sensing challenges and the corresponding machine learning techniques that have been proved to work well in practice. The table is meant to be a starting point for mobile sensing practitioners, and does not imply that alternative techniques would not perform better. The structure of the problem at hand often hints towards an efficient classification approach. For example, Gaussian Mixture Models perform well when it comes to speaker identification, as it is possible to extract parameters for a set of Gaussian components
from the FFT of the speech signal and use them as a vectorial representation of human voice. This approach has been proved extremely effective for user identification~\cite{reynolds2000}. However, a deeper discussion about why certain approaches work in certain domains is outside of the scope of this survey.

%Thus, phenomena that exhibit smooth transitions among states are naturally modelled by Markov chains. 
%Daily movement of a person often includes visits to the same set of places, e.g. home, work, school, in a well defined order. Time series analysis proves to be a suitable technique in this domain \cite{Scellato2011,DeDomenico2012}. 
Irrespective of the domain, in machine learning, data is king. A simple classifier built upon a large amount of data usually outperforms even the most complex classifier trained with insufficient information. Moreover, the amount of training data at our disposal determines the optimal classifier. Therefore, Naive Bayesian classifier usually performs well even with little data, as each feature can be independently estimated as a one dimensional distribution. This helps alleviate problems stemming from the curse of dimensionality, i.e., the need for data sets that scale exponentially with the number of features. More elaborate classification algorithms such as support vector machines (SVMs)~\cite{Cristianini2000} require more training data. Further, Forman and Cohen show that classifier performance depends on the distribution of classes in the training data set. This impacts both model selection as well as  feature selection, as different combinations of features and classifiers work best for different training data sets~\cite{Forman2004}.

\begin{table}%[htb]
%\figsp
\caption{Context sensing domains and relevant machine learning techniques.}
\label{tab:learners}
\begin{center}
\begin{scriptsize}
\begin{tabular}{|c|l|}
\hline
\textbf{Domain} & \textbf{Machine learning technique} \\
\hline
\hline
Speech recognition & 
\begin{tabular}[l]{@{}l@{}} -- Hidden Markov Model (HMM)\\ \cite{Chon2012,Choudhury2003}\\-- Threshold based learning \cite{Wang2009}\\-- Gaussian Mixture Model (GMM) \cite{Rachuri2010,Lu2012}\end{tabular}\\
%Complex: a function of locally relevant content, language and supporting infrastructure & Yes 
\hline
Activity classification & 
\begin{tabular}[l]{@{}l@{}}-- Boosted ensemble of weak learners\\ \cite{Consolvo2008,Abdullah2012}\\
-- Boosting \& HMM for smoothing \cite{Lester2005}\\-- Tree based learner \\  \cite{Tapia2007,Abdullah2012}\\-- Bayesian Networks~\cite{Krause2006}\end{tabular}\\
\hline
Location determination (with GPS) & 
\begin{tabular}[l]{@{}l@{}}-- Markov chain \cite{Ashbrook2003}\\
-- Non-linear time series \\ \cite{Scellato2011,DeDomenico2012}\end{tabular}\\
\hline
Location (with BT or WiFi) & \begin{tabular}[l]{@{}l@{}} -- Bayesian network\\
\cite{Eagle2006,Eagle2009a}\end{tabular}\\
\hline
Location (with ambient sensors) & -- Nearest neighbour \cite{Maurer2006}\\
\hline
Scene classification & -- K-means clustering \cite{Chon2012}\\
\hline
Object recognition & \begin{tabular}[l]{@{}l@{}}-- Support vector machine \cite{Chon2012}\\
-- Boosting \& tree-stump \cite{Wang2012}\end{tabular}\\
\hline
Place categorization & -- Labelled LDA~\cite{Chon2012}\\
\hline
Call prediction & -- Naive Bayesian \cite{Phithakkitnukoon2011}\\
\hline
Interruptibility & \begin{tabular}[l]{@{}l@{}}-- Bayesian Network \\ \cite{Horvitz2003,Fogarty2005}\\ -- Tree based learner \cite{Fogarty2005}\\
-- Naive Bayes~\cite{Hofte2007}\end{tabular}\\
\hline
\end{tabular}
\end{scriptsize}

\end{center}
\end{table}


%Data structure? 
%
%\begin{table}[htb]
%%\figsp
%\begin{center}
%\begin{scriptsize}
%\begin{tabular}{|c|l|}
%\hline
%\textbf{Domain} & \textbf{Characteristic Features} \\
%\hline
%\hline
%Speech recognition & 
%\begin{tabular}[l]{@{}l@{}} -- Sound spectral entropy, RMS, zero crossing rate, low energy frame rate,\\
% spectral flux, spectral rolloff, bandwidth, phase deviation\\
%\cite{Lu2009,Lane2011b}\\
%-- Mel-frequency cepstral coefficients (MFCCs)\\
%\cite{Lu2009,Miluzzo2010,Chon2012}\\
%\cite{Lu2010,Lu2012}\\
%-- Teager Energy Operator (TEO), pitch range, jitter and std. dev.,\\
%spectral centroid, speaking rate, high frequency ratio\\
%\cite{Lu2012,Lu2010}\\
%-- Running avg of amplitude, sum of abs differences\\
%\cite{Krause2006}\\
%-- Perceptual linear predictive (PCP) coefficients\\
%\cite{Rachuri2010}\\
%-- Mean and std. dev. of DFT power\\
%\cite{Miluzzo2008}
%
%
%%MFCC, Teager Energy Operator (TEO), Pitch range, jitter and stdev, Spectral centroid, speaking rate, high frequency ratio Lu2012, Lu2010 (without TEO)
%%Running average of amplitude, SAD KRause2006
%%Sound: Spectral entropy, RMS, zero crossing rate, low energy frame rate,spectral flux, spectral rolloff, bandwidth, phase deviation Lu2009, Lane2011b
%%Speech: auto correlation, spectral entropy Choudhury2003
%%HMM + MFCC Chon2012
%%Music: GMM + MFCC Chon2012
%%MFCC - Miluzzo2010
%%Mean+ STDEV of DFT power Miluzzo2008
%%Perceptual linear predictive (PLP) coefficients  Rachuri2010
%
%\end{tabular}\\
%\hline
%Activity classification & 
%\begin{tabular}[l]{@{}l@{}}-- Accelerometer FFT principal component analysis (PCA)\\
%\cite{Krause2006}\\
%-- Acc. intensity/energy/mean\\
%\cite{Eston1998,Lu2010,Rabbi2011,Abdullah2012}\\
%-- Acc. variance\\
%\cite{Miluzzo2008,Lu2010,Rabbi2011,Aharony2011}\\
%-- Acc. peaks/mean crossing rate\\
%\cite{Miluzzo2008,Lu2010}\\
%-- Acc. spectral features
%\cite{Lu2009,Lu2010,Lane2011b,Rabbi2011}\\
%-- Acc. correlations\\
%\cite{Abdullah2012}\\
%-- Acc. frequency domain entropy\\
%\cite{Abdullah2012}\\
%-- Barometric pressure\\
%\cite{Rabbi2011}
%
%\end{tabular}\\
%\hline
%
%Location & 
%\begin{tabular}[l]{@{}l@{}}
%-- Days on which any cell tower was contacted, \\
%days on which a specific tower is contacted, \\
%contact duration, events during work/home hours\\
%\cite{Isaacman2011}\\
%-- Tanimoto Coefficient of WiFi fingerprints \\
%\cite{Chon2012}\\
%-- Eigenbehaviors - vectors of time-place pairs\\
%\cite{Eagle2009b}\\
%-- Hour of day, latitude, longitude, altitude, social ties\\
%\cite{DeDomenico2012}\\
%\end{tabular}\\
%\hline
%Object recognition & \begin{tabular}[l]{@{}l@{}}-- GIST features\\
%\cite{Chon2012}
%\end{tabular}\\
%\hline
%Gestures & \begin{tabular}[l]{@{}l@{}}-- Mean, max, min, median, amplitude, and\\
%high pass filtered values of acc. intensity and jerk;\\
%spectral features; screen touch location, slope, speed,\\
%strokes number, length, slope and location\\
%\cite{Coutrix2012}\\
%\end{tabular}\\
%\hline
%Physiological state & \begin{tabular}[l]{@{}l@{}}-- Galvanic skin response, heat flux,\\
%skin thermometer running average and sum of absolute differences\\
%\cite{Krause2006}\\
%\end{tabular}\\
%\hline
%Thoughts & \begin{tabular}[l]{@{}l@{}}-- Bandpass filtered neural signal from EEG\\
%\cite{Campbell2010}\\
%\end{tabular}\\
%\hline
%Call prediction & \begin{tabular}[l]{@{}l@{}}--  Call arrival and inter-departure time, calling reciprocity\\  \cite{Phithakkitnukoon2011}\\
%\end{tabular}\\
%\hline
%Interruptibility & \begin{tabular}[l]{@{}l@{}}-- User typing, moving, clicking, application focus, app. activity, \\
%gaze, time of day, day of week, calendar, acoustic energy, WiFi environment,\\
%\cite{Horvitz2003}\\
%-- Mean, energy, entropy and correlation of accelerometer data\\
%\cite{Ho2005}
%\end{tabular}\\
%\hline
%\end{tabular}
%\end{scriptsize}
%\caption{}%Summary of machine learning techniques.}
%\label{tab:features}
%\end{center}
%\end{table}
%
%%
%%Depression in Bipolar disorder: self-reported mood rating Moore200?
%%
%%Social contacts: work or not, time of day, Bluetooth environment Ealgle2006
%%
%%The following are done via regression:
%%
%%Health state: phone calls, SMSs, communication diversity, BT rpoximity, WLAN APs distribution, late-night, early-morning communication Madan2011.
%%
%%Political opinion change: time, political opinion, type of interaction, amount of interaction, self-reported relationship. Madan2011
%%
%%Thoughts:
%%bandpassed filtered neural signal from EEG Campbell2010
%%%
%%Physiology: galvanic skin response, heat flux and skin thermometer running average and sum of absolute differences. Krause2006
%
%%Gesture recognition:accelereometer and acc. jerk mean, max, min, median, amplitude, variance , also high-pass filitered values. Spectral analysis: important frequencies;
%%touch location, touch slope, touch speed, num strokes, stroke lengths and locations, slopes <-min max mean median,. amplitude of all the above Coutrix2012
%%
%%Call prediction: call arrival time, interdeparture time, calling reciprocity Phithakkitnukoon2011
%%Interruptibility: whether a user is typing, moving or clicking with the mouse, current focus, application used, application activity, gaze, windows switching, opened windows, time of day, day of the week, if a meeting exists, acoustic energy, user location as determined with WiFi Horvitz2003
%%mean, energy, entropy and correlation of accelerometer data Ho2005
%
%%Activity Accelerometer FFT + PCA Krause2006; accelerometer intensity Eston1998; accelerometer variance Aharony2011
%%Energy, mean, variance and spectral features of the accelerometer + variance and signed change in pressure over various time windows for barometric pressure data Rabbi2011
%%Mean, variance, mean crossing rate, spectrum features of accelerometer Lu2010
%%Mean, energy, freq-domain entropy, correlation of accelerometer Abdullah2012
%%Mean, STDEV, num of peaks of acceleremeter Miluzzo2008
%%
%%Voice: Stress: MFCC, Teager Energy Operator (TEO), Pitch range, jitter and stdev, Spectral centroid, speaking rate, high frequency ratio Lu2012, Lu2010 (without TEO)
%%Running average of amplitude, SAD KRause2006
%%Sound: Spectral entropy, RMS, zero crossing rate, low energy frame rate,spectral flux, spectral rolloff, bandwidth, phase deviation Lu2009, Lane2011b
%%Speech: auto correlation, spectral entropy Choudhury2003
%%HMM + MFCC Chon2012
%%Music: GMM + MFCC Chon2012
%%MFCC - Miluzzo2010
%%Mean+ STDEV of DFT power Miluzzo2008
%%Perceptual linear predictive (PLP) coefficients  Rachuri2010
%%
%%Location (with BT or WiFi): eigenbehaviors - vectors of time-location pairs Eagle2009
%%Tanimoto Coefficient of WiFi fingerprints Chon2012
%%Location with cell towers: days on which any cell tower was contacted, days on which a specific tower is contacted, contact duration, events during work and home hours: Isaacman2011
%%
%%Object recognition: GIST features (FIND REF!) Chon2012
%
%The above discussion shows that numerous features can be extracted from a single modality. In many domains, however, certain feature types have crystallized out as the most informative. Table~\ref{tab:features} lists the most commonly observed features and the domains in which they are used. The table is not meant to be a comprehensive survey of feature extraction, but should point out that even with a small number of sensors there can be hundreds of possible features all of which may or may not contribute to context inference~\cite{Choudhury2008}. To tackle the problem of feature selection one possibility is to employ computationally inexpensive mathematical transformation known as the Principle Component Analysis (PCA)~\cite{Pearson1901}, as demonstrated in~\cite{Krause2006}. After the PCA is performed we are left with a set of most promising features that impact the target variable the most, i.e., in this case the aspect that we want to infer. However, different classifiers might give different results even with the same features. Wrapping is used as a more accurate, albeit more computationally complex, alternative to PCA~\cite{Kohavi1997}. In this procedure, based on the collected data, a classifier is built with each of the subsets of features. A part of the data is left out during the training phase and is used to evaluate the classifiers. An example of wrapping based feature selection can be found in the human interruption study by Fogarty et al.~\cite{Fogarty2005}. A boosting-based technique for ranking features according to their contribution towards context recognition has been proposed by Lester et al.~\cite{Lester2005}. Their approach iteratively trains an ensemble of weak binary classifiers constrained to use a single feature each. At the end of the training we are left with not only the ranking of features, but also with the weights that indicate how important each of the features is for the final classification. Interestingly, the same classifier, used in different environments, may require different features for successful classification. For example, Lu et al. find that a standard speech classification attribute MFCC does not perform well outdoors while more noise tolerant features, such as high frequency energy ratio and frequency centroid become more discriminative in this setting~\cite{Lu2012}.
%
%Modality and feature selection impact the rest of the context inference; a careful consideration at this stage of the process can help improve classification accuracy or reduce the computational complexity of the learning process. With an increasing number of sensors and a growing interest in a variety of context domains, identifying and quantifying the strength of a link between a domain and a modality or a feature emerges as an important research direction in mobile sensing.
%%Unfortunately, in many domains we still cannot answer a question of whether a link between a concept and a modality or a feature can be established.\mm{This comment might sound a bit vague - perhaps add more details}
%
%
%\subsubsection{Classification Methods}
%\label{sec:classification_methods}
%The construction of models is a crucial part of the design of context inference systems. A plethora of machine learning techniques at our disposal can be used to transfer distilled sensor data into mathematical representations of user behaviour. In this survey we concentrate on a small subset of machine learning techniques that have been successfully applied to mobile sensing problems, and we refer an interested reader to machine learning texts such as, for example,~\cite{Bishop2006,elementsstatisticallearning2009,RG11:first,Bar12:Bayesian}.
%
%We examine how context inference models are built in case of StressSense, mobile phone application that analyses speech data collected via a built-in microphone and identifies if a user is under stress \cite{Lu2012}. The first step in StressSense is sound and speech detection. The application assumes that sound is present if high audio level is present in at least 50 out of 1000 samples taken within a half a second period. In such a case, StressSense divides the audio signal into frames and for each of the frames calculates its zero crossing rate (ZCR) and root mean square (RMS) of the sound. These features correspond to sound pitch and energy. A tree-based classifier that decides between speech and non-speech frames is built with ZCR and RMS as attributes. Further, thresholds on ZCR and spectral entropy are used to discern between voiced and unvoiced frames of human speech. Finally, Gaussian Mixture Models (GMMs) are built for the two target classes -- stressed speech and neutral speech. Pitch, Teager Energy Operator (TEO) and Mel-Frequency Cepstral Coefficient (MFCC) based features of each voiced frame are used for user stress inference.\vp{Added example, consistent with the previous subsection that also has an example.}
%
%Thus, extracting Mel-Frequency Cepstral Coefficients and employing Gaussian Mixture Models has crystallized out as the most promising approach to sound classification~\cite{Lu2009, Rachuri2010, Miluzzo2010, Chon2012}, while tree-based classification or boosted ensemble of weak classifiers successfully tackle physical activity classification from accelerometer readings~\cite{Lester2005, Tapia2007, Miluzzo2008, Rabbi2011}.  

\subsubsection{Handling Large-Scale Inference}
\label{sec:large_scale}

Mobile sensing is moving from modelling behaviour of a small group of test users to observations of large populations. A recent trend is for mobile sensing applications to be distributed through commercial app stores such as Apple App Store and Google Play~\cite{Lathia2013b,Miluzzo2008}. Consequently, researchers sacrifice the comfort of being able to physically interact with study subject for the ability to gather larger, more diverse data. Novel challenges with respect to sensing application distribution, data processing and scalable machine learning have emerged. Data diversity calls for more complex classification: walking performed by an eighty year old person will yield significantly different accelerometer readings than when the same activity is performed by a twenty year old. Clearly, activity classification needs to be less general, but does that imply a personal classifier for each user? 

In~\cite{Lane2011a} Lane et al. propose community similarity networks (CSNs) that connect users who exhibit similar behaviour. User alikeness is calculated on the basis of their physical characteristics, their lifestyle and from the similarity between their smartphone-sensed data. For each of these three layers in the CSN, a separate Boosting-based classifier is trained for any individual user. However, a single-layer classifier is trained on the data coming from not only the host user, but also from all the other users who show strong similarity on that CSN layer. In this way the CSN approach tackles the shortage of labelled data for the construction of personalized models, a common issue in mobile sensing.

Besides increased user diversity, modern mobile sensing applications often put an emphasis on long-term observations. In their ``social fMRI'' study Aharony et al. gather over 25 sensing modalities continuously for more than a year from about 130 participants \cite{Aharony2011}. Machine learning algorithms need explicit labelling of the high level concepts that are extracted from sensor readings. However, with highly multi-modal sensing integrated with everyday life, querying users to provide descriptions of their activities becomes an intrusive procedure that may annoy them. Instead, a semi-supervised learning technique called \textit{co-training} is used to establish a bond between those sensor readings for which labels exist, and those for which only sensor data are present~\cite{Zhu2009}. Co-training develops two classifiers that provide complementary information about the training set. After the training on the labelled data, the classifiers are iteratively run to assign labels to the unlabelled portion of the data. In the mobile realm, unlabelled data representing an activity of one user could be similar to labelled data of the same activity performed by another user. In this case, labels can propagate through the similarity network of users~\cite{Abdullah2012}. 

In addition to a larger user base and an increased amount of gathered data, mobile sensing is further challenged by a growing number of devices used for context-aware applications. We increasingly observe \textit{ecosystems of devices}, where multiple devices work together towards improved context sensing. Fitbit, for example, markets a range of wearable devices that track user metrics such as activity, sleep patterns, and weight \cite{Fitbit}. As the popularity of these devices grows we can expect that a single user will carry a number of context sensing devices. Darwin Phones project tackles distributed context inference where multiple phones collaborate on sensing the same event \cite{Miluzzo2010}. First, via a cloud infrastructure, phones exchange locally developed models of the target phenomenon. Later, when the same event is sensed by different phones, inference information from each of the phones is pulled together so that the most confident description of the event is selected.

\subsection{Recognising Internal States}
Mobile sensing is not limited to inferring directly observable physical activities. Social signal processing (SSP) has emerged as a new research domain where behavioural cues such as gestures, conversations, facial expressions, and others are inferred and interpreted by means of machine learning and artificial intelligence tools~\cite{Pentland08:honest,Vinciarelli2009}. These cues, termed social signals, can be automatically analysed to understand, but also to mimic natural human behaviour \cite{Vinciarelli2012}. Analysing and synthesising behaviour solely with modalities available to machines, usually cameras and microphones, is a very hard task. Restriction to a phone renders this problem even harder to solve, due to increased noise and rapid context change that stems from user mobility and phone placement. Still, sophisticated states of individual and group psyche are increasingly in the focus of recent research on behaviour sampling. For example, EmotionSense, discussed in Section \ref{sec:select_features}, relates the way words are uttered during human speech with emotions the person experiences at the moment~\cite{Rachuri2010}. Likewise, StressSense, that we touched upon in Section \ref{sec:classification_methods}, uses mobile phone's microphone to measure user's stress levels~\cite{Lu2012}. NeuroPhone concentrates on thought inference, and represents a system that integrates brain signal reading with a mobile phone~\cite{Campbell2010}. The main motivation for NeuroPhone are novel hands-free interfaces, but one can envision applications that build complex intelligence by merging user's thoughts with phone's sensing and computational resources.


With a wealth of sensors on a mobile phone, information about mood can be correlated with user's location or activity, and used to identify novel psychological relationships among these concepts. Indeed, smartphones have a potential to completely revolutionize the way experimental social science research is done, as in situ examination of user's behaviour can be performed via a phone \cite{Miller2012}. In \cite{deMontjoye2013} the authors analyse mobile phone logs and establish relationships between the descriptors of users' calls, contacts and movement, and personality traits. Records of the way a user interacts with a touchscreen, or the way he moves a phone around can help identify hard-to-monitor affective behaviour~\cite{Coutrix2012}. Examining Bluetooth encounters among phones carried by office workers can help measure sociability and improve productivity~\cite{Rachuri2011}. Mobile phones can be used to uncover a wealth of information about us: from socio-economic factors \cite{Lathia2012,Martinez2012}, over our mental and physical health \cite{Rabbi2011,MCMFP12:sensing} to our thoughts~\cite{Campbell2010}. We believe that mobile sensing will also have an increasing role in the emerging area of computational social science~\cite{Lazer2009}.



==> tex/context_prediction.tex <==
% context prediction: anticipatory mobile computing 
% - anticipatory sensing intro (oSec 3 intro)
% - predicting user mobility and behaviour 
% - ! extend with other predictions !

\section{Context Prediction: Anticipatory Mobile Computing }
\label{sec:context_prediction}

Mobile sensing applications do not end at the point where a strong relationship between events we are interested in and the corresponding smartphone sensor data is established. Information collected during the inference phase can also serve as a basis for prediction of future events. Powerful machine learning algorithms and fine-grained sensor data represent a foundation for emerging applications that deliver accurate personalized predictions of future events. In a transition that Campbell and Choudhury call \textit{from smart to cognitive phones}, we can expect smartphones to become proactive personal assistants that anticipate and react upon our actions based on patterns learnt from our daily life~\cite{Campbell2012}. Such smartphones have the potential to co-exist in a symbiosis with their users and narrow the mismatch between the technology and humanity. They will allow for users' movement and action anticipation; they will know when to attract user's attention and when to stay silent; and they will proactively manage energy and wireless resources. Finally, predictive smartphones will close the loop providing valuable feedback and information that will shape user's future behaviour~\cite{Lathia2013}.
% Examples include applications for behaviour change
%warn their owners of important events or potential hazards. 
%With such a personal assistant, people will no longer forget to pack books in the morning of a day that they will pass by a library, or be unprepared for a sudden job interview phone call.

%In~\cite{Horvitz2003}, the authors develop a framework for inferring user's workload in an office setting. Done before the smartphones era, in order to infer interruptibility the proposed framework utilizes an external camera and a microphone, along with the information about user's desktop computer usage. The authors define the \textit{cost of interruption}, a metric that indicates how much a user is willing to pay to avoid an annoying event/notification of a certain type in a certain state. In every moment a sum of the probability that a user is in a specific state\mm{this part is unclear - why do you consider a sum of probability here? which kind of probability we are talking about here?} multiplied by the cost of interruption at that state represents the expected cost of interruption. A Bayesian network is then constructed in which variables such as the presence of voice, user's head position and gaze, currently opened applications on a user's PC, are connected with the probability distribution of interruptibility. Besides the current state, the method also forecasts times when a low, medium, or high state of interruptibility will be reached. In addition, the model seeks to find lingering times in each of the states. For example, it can predict time when a low interruptibility state in which a user will stay for at least five minutes is going to be reached.\mm{maybe this part should be shortened. We need to make clear that this work is not about anticipatory mobile sensing. Perhaps we should also say why this is relevant for mobile sensing}

%In another early work Fogarty et al. investigate which sensors should be constructed in order to efficiently infer interruptibility \cite{Fogarty2005}. They embrace a \textit{Wizard of Oz} technique, where human subjects simulate sensors by manually coding information from audio and video recordings. Despite the approach that allows examination of sensors that are yet to be implemented in reality, the authors find that simple sensors often provide enough hints to discern if a user is interruptible or not. Thus, detection of speech in the room remains the most powerful indicator of a non-interruptible state. The authors employ Naive Bayesian and tree-based machine learning algorithms, along with correlation-based and wrapping feature selection methods. In all cases simple sensors such as a microphone, mouse and keyboard activity, and telephone engagement sensor, provide sufficient information in order to infer interruptibility. Fogarty et al. also examine how interruptibility models evolve with the amount of data and the number of users under study \cite{Fogarty2004}. The analysis shows that the model needs little bootstrapping data before it starts producing high accuracy inferences. Moreover, training data from another user can substantially improve inference when the original user's data is not yet available. Generalizability of the findings, however, should be treated with caution. Two office workers considered in the study might have similar attention patterns, but people who work in different environments might not. \mm{also this is not really about mobile sensing: it should be shortened in my opinion. We also need to make clear why this is relevant for the prediction of context}

%Fogarty et al. point out to an important property of interruption: it is not an one off process, but a negotiated process where the interrupter probes and backs off if the subject is not interruptible at the moment. Kapoor and Horvitz evaluate how annoying different probing strategies are for a subject under study \cite{Kapoor2008}. Decision-theoretic strategies that construct a predictive model about user's internal state\mm{what do you mean by "user internal state" here? This should be clarified}, compute the expected value of information and weight the costs and benefits of probing act more in synchrony with the actual user behaviour than strategies that generate probes for situations associated with the most uncertainty, or at random times. Finally, Kapoor and Horvitz point out that a successful strategy has to follow changes in context over time and adapt to them. They develop one such strategy that not only learns, but forgets concepts that do not get reinforced over time. Their approach is based on decision-theoretic active learning. More details can be found in~\cite{Kapoor2007}. Context ``drift'' has been observed in other human behaviour classification problems as well. In the call prediction system we mentioned earlier, the authors note that recent trends in calling behaviour tend to be more indicative of the future calls than the whole history of caller/callee's behaviour~\cite{Phithakkitnukoon2011}. %pointing out an important problem in behavior prediction - how to tackle concept drifts and incorporate forgetting in online machine learning.


%
%
%Mobile sensing applications do not end at the point where a strong relationship between events we are interested in and the corresponding smartphone sensor data is established. Information collected during the inference phase can also serve as a basis for prediction of future events. Powerful machine learning algorithms and fine-grain sensor data represent a foundation for emerging applications that deliver accurate personalized predictions of future events. In a transition that Campbell and Choudhury call \textit{from smart to cognitive phones}, we can expect smartphones to become proactive personal assistants that anticipate and react upon our actions based on patterns learnt from our daily life~\cite{Campbell2012}. Such smartphones have the potential to co-exist in a symbiosis with their users and narrow the mismatch between the technology and humanity. They will allow for users' movement and action anticipation; they will know when to attract user's attention and when to stay silent; and they will warn their owners of important events or potential hazards. Finally, predictive smartphones will close the loop providing valuable feedback and information to users. Examples include applications for behaviour change~\cite{Lathia2013}.
%%With such a personal assistant, people will no longer forget to pack books in the morning of a day that they will pass by a library, or be unprepared for a sudden job interview phone call.
%
%\subsection{Improving Human-Computer Interaction Through Anticipatory Sensing}
%\label{sec:improvingHCI}
%
%Context predictions enabled through mobile sensing can serve as a basis for device's adaptation to its owners' lifestyle. Mobile phones are used in a highly personalized context and a need arises for their customized interaction with individual users. Basic personalization can came from explicit rules that a user sets, such as the assignment of speed dial numbers or ringer sounds. However, phone's ability to predict user behaviour allows seamless integration with user's daily routine. An example of a mobile phone system that anticipates, and adapts to user behaviour is the call predictor developed in~\cite{Phithakkitnukoon2011}. The authors devise an outgoing call predictor termed ``Incoming Call Forecast" and an outgoing call predictor, which they refer to as an ``Intelligent Address Book". The former can help people optimize their daily schedules, while the latter, by giving higher preference to those contacts that are more likely to be called, improves navigation through user's address book. For both purposes a probabilistic model that captures the caller's behaviour, the callee's behaviour, reciprocity between the two, and the behaviour trends is built. Calling times often exhibit daily periodic patterns, thus time-of-day and call inter-arrival times prove to be reliable features for building such a prediction model. 
%
%In his 1991 manifesto of ubiquitous computing Weiser advocates pervasive technology that coexists unobtrusively with its users \cite{Weiser1991}. This ``calm technology" is not our current reality, and indeed we get an abundance of notifications from an increasing number of devices we own. Thus, we receive irrelevant instant messages while working on an important project, a phone may sound an embarrassing ``out of battery" tone in the middle of a meeting, and a software update pop-up may show up while we are just temporarily connected to a hot spot in a coffee shop. 
%
%\textit{Attentive user interfaces} manage user attention so that the technology works in symbiosis with, rather than against user's interruptibility. Frameworks for inferring user's availability had been developed before the smartphones era. In~\cite{Horvitz2003}, relying on an external camera and a microphone, along with the information about user's desktop computer usage, the authors develop a framework for inferring user's workload in an office setting. A Bayesian network is then constructed in which variables such as the presence of voice, user's head position and gaze, currently opened applications on a user's PC, are connected with the probability distribution of interruptibility. In another early work Fogarty et al. investigate which sensors should be constructed in order to efficiently infer interruptibility \cite{Fogarty2005}. They embrace a \textit{Wizard of Oz} technique, where human subjects simulate sensors by manually coding information from audio and video recordings. Despite the approach that allows examination of sensors that are yet to be implemented in reality, the authors find that simple sensors often provide enough hints to discern if a user is interruptible or not. Thus, detection of speech in the room remains the most powerful indicator of a non-interruptible state.
%
%The above interruption studies are of great importance in the field of experience sampling.  Experience sampling is a common research technique in psychology~\cite{Hektner2006} where users are asked to provide information about their current experiences in real time. Mobile devices revolutionized this research field, as they enable in-situ probing of users' daily lives. Specialized smartphone frameworks for experience sampling have been developed recently \cite{Froehlich2007,Rachuri2011,Ramanathan2012}. Still, assessing interruptibility remains an important problem, and, beyond isolated attempts, the area remains largely unexplored. 
%One of the most representative papers in this area is~\cite{Ho2005} by 
%Ho and Intille: in this work the authors
%show how an accelerometer can be used to infer activity transitions, period when, the authors argue, a user is more susceptible to interruption~\cite{Ho2005}. Accelerometer movement is just one of many modalities that modern smartphones can sense, and interruptibility prediction for social science experiments remains to be fully explored.
%
%- Fogarty 2005: Interruption is not a one off process. It is a negotiated process. We probe the interruption and back of if the person is not interruptible. 


\subsection{Predicting User Mobility, Actions and Behaviour}

Historically, prediction of mobile phone users' movement patterns was tied with system optimizations. Anticipation of surges in the density of subscribers in a cellular network was proposed for dynamic resource reservation and prioritized call handoff~\cite{Soh2003}. Yet, as data collected by a phone gets more personal, the opportunity for novel user-centric anticipatory applications increases. 

User movement can be examined on different scales. For small-scale indoor movement predictions, systems can rely sensors embedded in the buildings. An example of such systems is MavHome: the authors proposes a smart home which adjusts indoor light and heating according to predicted movement of house inhabitants~\cite{Cook2003}.  A large part of the current research, however, concentrates on the city-scale prediction of users' movement. Early on the extraction of significant places for the users got in the focus of mobility prediction research~\cite{Ashbrook2003,hightower2005}. The interest was further raised with proliferation of smartphones and commercial location-based services such as Foursquare \cite{Foursquare}. In such as setting, targeted ads can be disseminated to phones of users who are expected to devote a certain amount of their time to eating out or entertainment. The NextPlace project aims to predict not only user's future location, but also the time of arrival and the interval of time spent at that location \cite{Scellato2011}. The authors base the prediction on a non-linear time series analysis. More recently, Horvitz and Krumm devise a method for predicting a user's destination and suggesting the optimal diversion should the user want to interrupt his/her current trip in order to, for example, take a coffee break \cite{Horvitz2012}. Noulas et al. investigate next check-in prediction in the Foursquare network \cite{Noulas2012}. They show that a supervised learning approach that takes into account multiple features, such as the history of visited venues, their overall popularity, observed transitions between place categories, and other features, need to be jointly considered for a successful prediction. SmartDC merges significant location prediction with energy-efficient sensing, and proposes an adaptive duty cycling scheme to provide contextual information about a user's mobility \cite{Chon2013}.  SmartDC learns user mobility with an unsupervised learner, and builds a Markov chain that guides adaptive duty cycling of the GPS sensor. 

%These systems involve the prediction and classification of locations of multiple users performed locally on the device or in the back-end. For instance, intertwined movement patterns of multiple users in an urban scenario are exploited in the work by McNamara et al.~\cite{McNamara2008}. The authors propose a system for sharing media files among urban commuters who are expected to traverse the same route. A probabilistic reasoning framework for context-aware decisions for supporting drivers is presented in~\cite{Ziebart08}. The framework is built upon reinforcement learning algorithms based on the analysis of the preferred routes of the drivers. The evaluation of this work is performed on the collection of mobility traces of 25 taxi drivers over 3 months.
GPS is not the only modality that can be used for mobility prediction. 
%Mobile sensing for location prediction does not need to be limited to GPS coordinate tracking. 
Supplementing and substituting GPS coordinates with phone's accelerometer readings has been proposed for improving energy efficiency of location prediction \cite{Zhuang2010,BenAbdesslem2009}. Moreover, additional context can increase the accuracy of prediction. Thus, SurroundSense utilizes audio and video sensors to assign an audio-visual fingerprint to a location \cite{Azizyan2009}. 

Research on mobility prediction was additionally boosted by large sets of multimodal data that have been collected and made publicly available by companies and academic institutions. For example, the MIT Reality Mining~\cite{Eagle2006} project accumulated a collection of traces from one hundred subjects monitored over a period of nine months. Each phone was preloaded with an application that logged incoming and outgoing calls, Bluetooth devices in proximity, cell tower IDs, application usage, and phone charging status. Similarly, the Nokia Mobile Data Challenge (MDC) data set was collected from around 200 individuals over more than a year \cite{Laurila2012}. The logs contain information related to GPS, WiFi, Bluetooth and accelerometer traces, but also call and SMS logs, multimedia and application usage. The above data sets served as a proving ground for a number of approaches towards mobility prediction. In~\cite{Eagle2009a} Eagle et al. demonstrate the potential of existing community detection methodologies to identify significant locations based on the network generated by cell tower transitions. The authors use a dynamic Bayesian network of places, conditioned on towers, and evaluate the prediction on the Reality Mining data set. De Domenico et al. exploit movement correlation and social ties for location anticipation~\cite{DeDomenico2012}.  Relying on nonlinear time series analysis of movement traces that do not originate from the user, but from user's friends or people with correlated mobility patterns, the authors demonstrate improved accuracy of prediction on the MDC data set. Interdependence of friendships and mobility in a location-based social network was also analyzed in~\cite{Cho2011}. Finally, besides its expansion to cover larger user groups, the field of mobility prediction is also advancing towards broader prediction time horizons. Recently, it has been shown that, by extracting recurring patterns in human mobility, predictions can go even months into the future~\cite{Sadilek2012}.

Multimodal traces also enabled activity or behaviour prediction. Human activity recognition has been an active subject of research in the past years: various approaches have been presented in the literature, based for example on accelerometer~\cite{Choudhury2008,Tapia2007}, state-change sensors \cite{Tapia2004} or a system of RFIDs \cite{Wyatt2005}. In a series of seminal works such as~\cite{LFK05:Liao,liao2007hcr}, Liao et al. demonstrate the prediction and correlation of activities using location information. Eagle and Pentland propose the use of multimodal \textit{eigenbehaviors}~\cite{Eagle2009b} for behaviour prediction. Eigenbehaviors are vectors that describe key characteristics of observed human behaviour over a specified time interval. The vectors are obtained through the principal component analysis (PCA) of a matrix that describes a deviation in sensed features. Besides being a convenient notation for time-variant behaviour, by means of simple Euclidean distance calculation, eigenbehaviors enable direct comparison of behaviour patterns of different individuals. Eagle and Pentland demonstrate the ability of eigenbehviors to recognize  structures in behaviours by identifying different student groups from the Reality Mining data set. 

%The exploitation of location information together with other sensor data is an active and very promising research area. 
Anticipatory sensing enables inference of subtle characteristics of human behaviour. In their work on health status prediction, Madan et al. use mobile phone based co-location and communication sensing to measure characteristic behaviour changes in symptomatic individuals~\cite{Madan2010}. The authors find that health status can be predicted with such modalities as calling behaviour, diversity and entropy of face-to-face interactions and user movement patterns. Interestingly, they demonstrate that both physiological as well as mental states can be predicted by the proposed framework. 

Rich psychological context, including user's expectations, cognitive load and flexibility in decision making can be harnessed in mobile computing applications~\cite{Bao2013}. Bao et al. show that various domains, such as image compression and video streaming can benefit from psychological context inference. Finally, political opinion fluctuation is a topic of another pioneering work by Madan et al.~\cite{Madan2011a}, which show the potential use of the information collected by mobile sensing systems for understanding and predicting human behavior at scale. In this work call and SMS records, Bluetooth and WiFi environment and  are used to model opinion change during the 2008 presidential elections in the United States. Face-to-face personal encounters, measured through Bluetooth and WiFi collocation, are the key factor in opinion dissemination. The authors also discover patterns of dynamic homophily related to external political events, such as election debates. Automatically estimated exposure explains individual opinions on election day. 

Finally, anticipatory mechanisms can be used to improve the performance of mobile systems themselves, such as pre-launching applications that are going to be used. For example, the FALCON system predictively prelaunches apps based on context signals and user access patterns. Prelaunch includes both preloading mobile apps in memory and fresh content preparation for the specific application, such as prefetching email in case of email clients~\cite{yan2012fast}.

% Non-linear time series analysis is also used by De Domenico et al who exploit movement correlation and social ties for location anticipation \cite{DeDomenico2012}. Harnessing movement traces from users' friends or people with correlated mobility patterns, the authors demonstrate improved accuracy of prediction on the MDC data set.


